Adaptive Neural Network-Based Approximation to Accelerate Eulerian Fluid Simulation

The Eulerian fluid simulation is an important HPC application. The neural network has been applied to accelerate it. The current methods that accelerate the fluid simulation with neural networks lack flexibility and generalization. In this paper, we tackle the above limitation and aim to enhance the applicability of neural networks in the Eulerian fluid simulation. We introduce Smartfluidnet, a framework that automates model generation and application. Given an existing neural network as input, Smartfluidnet generates multiple neural networks before the simulation to meet the execution time and simulation quality requirement. During the simulation, Smartfluidnet dynamically switches the neural networks to make the best efforts to reach the user requirement on simulation quality. Evaluating with 20,480 input problems, we show that Smartfluidnet achieves 1.46x and 590x speedup comparing with a state-of-the-art neural network model and the original fluid simulation respectively on an NVIDIA Titan X Pascal GPU, while providing better simulation quality than the state-of-the-art model.

==> Content/draft.tex <==
%\textcolor{dong}{we predict $CumDivNorm^{final}$ at each time interval. At a time interval, to predict $Q_{loss}$, we check $CumDivNorm^{final}$ in the previous time intervals and find $k$ time intervals whose  $CumDivNorm^{final}$ are the closest to $CumDivNorm^{final}$ in the current time interval. We use the average of $Q_{loss}$ in the $k$ time intervals as the predicted $Q_{loss}$ in the current time interval.}
%given a set of predicted pairs in the middle of the fluid simulation, we choose $k$ pairs, whose $CumDivNorm^{final}$ is closest to the predicted $CumDivNorm^{final}$. 
%given the predicted $CumDivNorm^{final}$ in the middle of the fluid simulation, we choose $k$ pairs, whose $CumDivNorm^{final}$ is closest to the predicted $CumDivNorm^{final}$. We use the average  of the $Q_{loss}$ in the $k$ pairs as the predicted $Q_{loss}$.
%\textcolor{dong}{The above sentence is confusing. We need to discuss.}
%Eulerian Fluid Simulation is a particularly effective formula of modeling hydrodynamics in many physical applications. High computational complexity of traditional iterative solvers leads to limited deployment, while several neural network-based methods greatly reduce the labor of computation by learning complicated relationships between input and output datasets and draw wide attention. However, these state-of-the-art methods apply single network topology to this input-sensitive application, thus resulting in the inability to achieve required accuracy or the inefficiency to leverage the power of deep learning.

%In this work, we propose Smart-fluidnet framework, which provides various approximate models and enables adaptive approximation to accelerate Eulerian Fluid Simulation for arbitrary user requirements and input samples. For this purpose, we generate multiple flexible and comprehensive network topologies by improved model transformation and select the most suitable candidates by designed offline output-quality controller, then a quality-aware runtime algorithm dynamically singles out the optimal one with negligible overhead.
%We evaluate our work on an NVIDIA Pascal GPU, and results show that Smart-fluidnet is on average 1.1x and 1.71x faster than Tompson's method with the grid size of 256*256 and 1024*1024.

%The Eulerian fluid simulation is an effective method of modeling fluid in many HPC applications. The high computational complexity of traditional solvers leads to limited deployment of this , while several neural-network-based methods reduce the labor of computation by learning complicated relationships and draw wide attention. However, these state-of-the-arts apply single network topology to this input-sensitive application, resulting in inability for achieving required accuracy or inefficiency for leveraging the power of machine learning.

\begin{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth, ]{Figures/sec4_dropout.pdf}
       \vspace{-10pt}
        \caption{Quality losses of Five different MLPs. %\textcolor{green}{Change the x axis title to "Grid size"}
        } 
  \vspace{-15pt}
  \label{fig:dropout_loss}
\end{figure}
\end{comment}
%\textcolor{dong}
%if the time step of the currently selected model is less than five, we skip the first five to make sure the trend is stable and only use the following five to build the model. Then if the predicted $CumDivNorm^{final}$ of the currently selected model is close to user requirement, we continue to collect the next five steps for the next regression. But we will also skip the first five steps for possible model conversion. %Approximate computing also receives many attentions recently. It has been applied in many areas, such as hardware acceleration~\cite{Esmaeilzadeh:2012:ASD:2150976.2151008, 6569370, Ranjan:2014:ASA:2616606.2617119, Sampson:2013:ASS:2540708.2540712}, compiler optimization~\cite{baek2010green, Misailovic:2010:QSP:1806799.1806808, Sampson2015ACCEPTAP, sidiroglou2011managing}, programming language designs~\cite{5523464, Rinard:2006:PAB:1183401.1183447, samadi2013sage, Sampson:2011:EAD:1993498.1993518}, and runtime systems~\cite{Campanoni:2015:HRP:2738600.2738630, Goiri:2015:ABA:2694344.2694351, Hoffmann:2011:DKR:1950365.1950390}.
%So this approach significantly improves the performance by smoothing the input of the problem, but the data dependency make it difficult to be parallelized on GPUs.
%Based on the potential of using DNNs to approximate computation in the fluid simulation and the fluid simulation can be processed as a supervised regression problem, %However, these research did not provide a systematic approach to construct neural networks for fluid simulation. The way of constructing neural networks to meet the user’s requirement on execution time and simulation quality is not be solved. Our proposed framework aims to address these limitations in the fluid simulation scenario to some certain extent.
%\textcolor{wq}{Our work also resembles the recent model compression, which aims to reduce the parameter sizes of neural networks~\cite{cheng2017survey}. To achieve smaller network models, model compression includes various methodologies, e.g., quantization parameters~\cite{jacob2018quantization,wu2018training}, layer pruning~\cite{yang2017designing,molchanov2016pruning}, binarized networks~\cite{rastegari2016xnor,courbariaux2016binarized}, low rank approximation~\cite{tai2015convolutional}, or knowledge distillation~\cite{sau2016deep,lopes2017data}. While these methods typically focus on generalized model compression tasks with limited resources, our proposed algorithm makes guarantees on specific user input requirements.}%%reach the user requirement. 
%%smart-fluidnet uses an MLP-based model to select the most promising neural network models that could meet the user requirement on performance (execution time) and simulation quality. 
%by offline output-quality control. 
%first dynamically chooses some approximation models that be used to minimize the possibility of violating user requirement based on predicted output quality.
%%%\noindent\textbf{Approximation model construction.} %Based on a basic CNN model, Smart-fluidnet takes Auto-Keras as a plugin and extends its function to generate effective approximate models by Pareto optimality.  For this propose, 
%%%we design four operations (deleting, narrowing, pooling and dropout) to transform the input neural model to simpler ones. Then we choose neural network models that are promising for performance improvement and high quality based on the Pareto optimality analysis. %multiple flexible and comprehensive network topologies for maximizing coverage of the \textit{Appr. (Approximate) Model Pool}.

%%%\noindent\textbf{Offline output-quality control.} Given the user requirement on simulation quality and execution time, the \textit{MLP-based quality controller} selects the most promising approximate models from the \textit{Appr. Model Pool}. %The MLP-based model collects some statistical data from the training phase of approximate models. \textcolor{blue}{Then in order to improve the efficiency for selecting suitable models, the MLP-based model constructs a success possibility for each available approximate model by evaluating whether the final quality loss and execution time are met and is trained offline without extra runtime overhead. } 

%%%\noindent\textbf{Quality-aware runtime design.}  For a large number of input problems, a single neural network-based approximation model may not meet various user requirements or exhibit too excessive accuracy to squander more calculation time. As the main runtime component in the framework, quality-aware runtime design makes full use of the advantages of multiple approximation models and dynamically selects the optimal one with the minimum amount of calculation under the premise of satisfying user requirements. 

%
%%The main advantage is that the smart-fluidnet framework combines user requirements, sample characteristics, and neural network models together to search the optimal matching solution. Next, we will begin to introduce the three components in details.%{The new neural network models can be more accurate than the input model; They can be also less accurate than the input model. Having such a mixture of different models provides flexible computation approximation during the online fluid simulation.}
%\textcolor{dong}%\textcolor{dong}
%\textcolor{wq}{Why list these explanations here????}
%{We generate less accurate models using the following methods.} Previous work on neural network transformation is mainly based on two methods: layer-level~\cite{cai2018path} and graph-level transformation~\cite{bottou2005graph}. The layer-level transformation preserves the functionality of the layers. However, this method breaks the consistency of input and output tensors in the neural network. The graph-level transformation addresses this problem. This method changes the architecture of the input neural network by transformation operations. Those operations either make the network deeper or widen the intermediate layers of the neural network. 
%As a result, the new neural network is more computation intensive which leads to longer execution time. Thus, the existing transformation operations are not enough in our application. %\textcolor{wq}{This operation reduces the number of the model parameters, thus decreasing the accuracy of predictions.}%\textcolor{wq}{Similar to operation 1, this operation also reduces the number of the model parameters, but it maintains the depth of the model.}%\textcolor{dong}{This operation is useful to increase the receptive field of the final output features.}
%\textcolor{wq}{This operation also reduces the number of parameters but it increases the receptive field of the final output features.}
%\textcolor{wq}{Each operation introduces unique characteristics (such as increasing receptive field, increasing generalization capability, etc) while reducing the complexity of network typologies. These unique characteristics has different level of importance depending on the states of current model. There is no systematic ways to determine which combination is the most efficient (reducing network redundancy without heavily hurting accuracy). Hence, a predefined order of using these operations by users is inevitable in network simplification. We follow a rule that an operation which reduces more neurons than others will be conducted earlier. We conduct four transformation operations sequentially and our model transformation algorithm works as follows.}
%Figure~\ref{fig:sec7_2} shows the results of the quality loss for all input problems with five grid sizes. For each case, the figure shows a box bounding by 25th and 75th percentiles of the quality loss; The central mark of the box indicates the median; the `+' markers outside the box indicates the extreme outliers~\cite{dawson2011significant}. %(1) In all cases, the boxes for Smart-fluidnet are smaller than the corresponding ones for the Tompson's model; (2) The numbers of extreme outliers with Smart-fluidnet are smaller than those with the Tompson's model.

%The two observations reveal that Smart-fluidnet can give more \textit{consistent simulation quality} than the Tompson's model, when given various input problems. The simulation quality with Smart-fluidnet is also higher than that with the Tompson's model. Having a consistent simulation quality is important to meet the user requirement on the simulation quality.%, using the performance of PCG as the baseline.%$1.46 \times$ speedup.
%On average, Smart-fluidnet performs $1.46 \times$ better than the Tompson's model. 
%\textcolor{wq}{There is no overlapping between the training and test datasets. To generate the 40,960 problems, we initialize velocity in a pseudo-random turbulent field\cite{kim2008wavelet}, and generate occupancy grids with border wall by introducing some objects in simulation domain. These objects are from the NTU 3D Model Dataset~\cite{pu2006visual}. }
%when using all input problems for the fluid simulation with the Tompson's model, as the user requirement (the target).%The evaluation frequency is a parameter in our runtime algorithm (see Section~\ref{sec:lightweight predictor}). The evaluation frequency decides how often the runtime system evaluates (predicts) whether the current neural network model can reach the user requirement on the simulation quality.
%\textcolor{wq}{Figure~\ref{fig:sec7_7} shows that the success rate drops quickly when the interval is larger than 8, and it continually decrease when the interval increase. We observe a abrupt performance growth at the check interval 16, which should be attributed to the large variation of low evaluation frequency. Due to the variance of evaluated input problems, the long check frequency may miss the timing of switching neural networks for the simulation, thus causing some fluctuations in the success rate v.s. check interval plot. Since evaluation frequency affects the prediction accuracy, the long evaluation interval bring in the large variance of prediction. }

%\textcolor{wq}{We study the computation and memory overhead about introducing neural networks.We evaluate the resource usage by PCG, Thompson and our proposed method with the grid size of 512*512. The results are presented in Table~\ref{tab:workload}.  From the table, we find that the Tompson consumes less memory than PCG. While Smart-fluidnet  requires much more memory than PCG and Tompson. However, our GPU devices are equipped with sufficient large memory, so memory usage by our algorithm is acceptable. On the other hand, Smart-fluidnet requires much less FLOPS than Tompson on average for a single step. This is because, we use small convolutional networks than Tompson for  most of the input problems.}
%
% The "title" command has an optional parameter, allowing the author to define a "short title" to be used in page headers.
%
% The "author" command and its associated commands are used to define the authors and their affiliations.
% Of note is the shared affiliation of the first two authors, and the "authornote" and "authornotemark" commands
% used to denote shared contribution to the research.

%
% By default, the full list of authors will be used in the page headers. Often, this list is too long, and will overlap
% other information printed in the page headers. This command allows the author to define a more concise list
% of authors' names for this purpose.

%\textcolor{wq}{To solve Equations \ref{equ:NS_momentum} and \ref{Equ:Possion_equation}, we use standard operator spitting method to split into three parts, i.e., advention step, external force step, and pressure projection step. The basic Eulerian procedure is shown in Algorithm \ref{Eulerian algorithm}.}
%Velocity and pressure update applies to every velocity component that borders a grid cell that contains fluid. The pressure in a grid cell is sampled at the centre of the cell and the velocity is sampled at the centers of the vertical cell faces. With this staggered arrangement, we can get unbiased second-order accuracy of a central difference without a null-space problem, and it simplifies the solid-cell boundaries condition handling.}
%and then substitute Equation~\ref{Equ:incompressibility_condition} as one part to satisfy stability.  %Mantaflow uses the Eulerian method (a method for computational fluid dynamics) which includes the above three parts. 
%\textcolor{wq}{To solve Equations~\ref{equ:NS_momentum} and~\ref{Equ:incompressibility_condition},  we use standard operator spitting method to split up equations into three parts and solve each one separately in turn. The three parts include  advection, adding external force, and pressure projection. Algorithm~\ref{Eulerian algorithm} shows the basic Eulerian framework.}

 %Weighting term $w_i$ is used to emphasize the importance of fluid-solid border conditions since the border is crucial to the simulation stability. 
%\textcolor{wq}{$DivNorm$ in Equation~\ref{Equ:Objective_function} is the sum over all fluid cell (mesh volumes) in the rendered smoke frame.}
%\textcolor{wq}{In this equation, $w_i$ is a per-vertex weighting term that emphasizes the divergence of grids on geometry boundaries, i.e., $w_i = max(1,k-d_i)$, where $d_i$ is a distance field with value 0 for solid cells or the minimum Euclidean distance of each fluid-cell to the nearest solid cell. Weights are used to emphasis the importance of fluid-solid border conditions since the border only represents a small fraction of the whole domain but crucial to the simulation stability.}

%Fluid simulation aims to study the flow of fluid materials and has been widely applied to multiple disciplines. The neural network, as a tool to learn and model complicated (non)linear relationships between input and output datasets, has been applied to accelerate the Eulerian fluid simulation. The current methods to accelerate the fluid simulation using neural works have fundamental limitations, because of the lack of flexibility and generalization; Also, there is no systematic approach to construct and apply neural network models for the fluid simulation.
%
% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% Please copy and paste the code instead of the example below.
%

%
% Keywords. The author(s) should pick words that accurately describe the work being
% presented. Separate the keywords with commas.
%\keywords{Machine learning, Quality control,}

%
% This command processes the author and affiliation and title information and builds
% the first part of the formatted document.

%In this paper, we tackle the above limitations and aim to enhance the applicability of neural networks in HPC applications (particularly the Eulerian fluid simulation). We introduce Smart-fluidnet, a framework that automates the model generation and application. Given an existing neural network model as input, Smart-fluidnet generates multiple neural network models before the simulation to meet the requirement on execution time and \textcolor{red}{simulation quality}. During the simulation, Smart-fluidnet dynamically switches the neural network models to make best efforts to reach the user’s requirement on simulation quality. Evaluating with 20,480 input problems, we show that Smart-fluidnet is 46\% and 590x faster than the Tompson's model (the state-of-the-art neural network model) and the original fluid simulation respectively on an NVIDIA Pascal GPU without violating the requirement on simulation quality.


%which provides various approximate models and enables adaptive approximation to accelerate fluid simulation. We generate multiple network typologies by designed transformation operations and select the most suitable models by offline output-quality controller, then a quality-aware runtime algorithm dynamically singles out the optimal one with ignorable runtime overhead. The results show that Smart-fluidnet is 46\% and 590x faster than Tompson's method (the state-of-the-art neural network model) and original fluid simulation respectively on an NVIDIA Pascal GPU.

%In Algorithm~\ref{Eulerian algorithm}, the advection procedure (Line 4) ignores the pressure term ($- \bigtriangledown p$) and returns an approximation to the result of advecting the field quantity $q$ through the velocity field $\vec{u}$. After that, the external body forces (Line 5) are added to the forward velocity of fluid. For the pressure projection, the algorithm first calculates the pressure (Line 7, solving an Poisson's equation) to make $\vec{u}_{n+1}$ divergence-free, and also enforces the solid wall boundary conditions~\cite{jeffrey2003applied} (i.e., $\vec{u}_{n+1}\centerdot \hat{n} = \vec{u}_{solid}\centerdot \hat{n}$). 


%\textcolor{dong}{In the above process, solving the Poisson's equation is the most crucial and time-consuming step to preserve the divergence-free constraint on the velocity and maintain simulation accuracy. The end of the pressure projection (Line 18) produces a divergence-free velocity field, $\vec{u}^{n+1}$, by subtracting the pressure gradient ($\Delta t \frac{1}{\rho} \bigtriangledown \vec{p}_n$) from the approximate velocity field $\vec{u_B}$}.


%\textcolor{wq}{In Algorithm~\ref{Eulerian algorithm}, the advection procedure(line 4) ignores the pressure term ($- \bigtriangledown p$) and returns an approximation to the result of advecting the field quantity $q$ through the velocity field $\vec{u}$.
%create an advect velocity field, which includes unwanted divergence. Add body forces part(line 5) are applied on the fluid to forward velocity with integrating external body forces. Pressure projection first calculates the right pressure (line 7) to make $\vec{u}_{n+1}$ divergence-free, and also enforces the solid wall boundary conditions\cite{jeffrey2003applied} (i.e., $\vec{u}_{n+1}\centerdot \hat{n} = \vec{u}_{solid}\centerdot \hat{n}$). Note that this is the most crucial step to prevent blow up and maintain simulation accuracy. And then, the project routine (Line 16) produces a divergence free velocity field, $\vec{u}^{n+1}$, by subtracting off the pressure gradient from the approximate velocity field $\vec{u_B}$}.

%\textcolor{wq}{During the advection, we introduce the semi-Lagrangian method~\cite{stam1999stable} to trace backward particle trajectory for the convection term and implicit solver for the viscosity and pressure terms. For pressure projection, by introducing the MAC grid, we discrete the solver space and come up with a system of linear equations. Each fluid grid cell is related to a linear equation to make the fluid incompressible. Integrating the whole solving space, it involves solving the following Poisson's equation (line 7):
%\begin{equation}
%   \bigtriangledown \cdot \bigtriangledown \vec{p} = \frac{1}{\bigtriangleup t} \bigtriangledown \cdot\  \vec{u}^*.
%   \label{Equ:Possion_equation}
%\end{equation}
%Rephrasing the above equation as $A\vec{p_t}=d$, A is referred to a symmetric positive semi-definite matrix, which usually takes a large number of iterations to let the equation converge to a small residual. One particularly useful algorithm for solving symmetric positive (semi-)definite linear systems is called the Conjugate Gradient algorithm, usually abbreviated as CG.}

%%%\textcolor{wq}{During the advection, we introduce the semi-Lagrangian method~\cite{stam1999stable} to trace backward particle trajectory for the convection term and implicit solver for the viscosity and pressure terms. For pressure projection, by introducing the MAC grid, we discrete the solver space and come up with a system of linear equations. Each fluid grid cell is related to a linear equation to make the fluid incompressible. Integrating the whole solving space, it involves solving the following Poisson's equation (line 7):
%At each time step, solving the following Poisson's equation(step 5) is the most computationally demanding component. 
%\begin{equation}
%   \bigtriangledown \cdot \bigtriangledown \vec{p} = \frac{1}{\bigtriangleup t} \bigtriangledown \cdot\  \vec{u}^*.
%   \label{Equ:Possion_equation}
%\end{equation}
%Rephrasing the above equation as $A\vec{p_t}=d$, A is referred to a symmetric positive semi-definite matrix, which usually takes a large number of iterations to let the equation converge to a small residual. One particularly useful algorithm for solving symmetric positive (semi-)definite linear systems is called the Conjugate Gradient algorithm, usually abbreviated as CG.
%This  symmetric positive (semi-)definite linear systems}
%The process of solving the Poisson's equation in mantaflow is based on the Preconditioned Conjugate Gradient (PCG) method, which involves large computation that iteratively converges to  meet convergence criteria (line 8-16) .\textcolor{wq}{We use a multi-grid approach\cite{mcadams2010parallel} as a preprocessing step of the PCG method. The precinditioner (line 10) applied in this paper is Modified Incomplete Cholesky L0 preconditioner, called “MICCG(0)”.} The existing work~\cite{tompson2017accelerating} and our work use a neural network to replace the PCG method.
%During the training process, the neural network operates on a few samples of data at a time called a \textsl{mini-batch}.  Many mini-batches are iteratively fed into the neural network for training.  %\textcolor{dong}{(TODO: Here, define what are positive training samples and negative training samples.)}
%In the fluid simulation, the computation domain is divided into grids with a Cartesian coordinate system. As a result, Equation~\ref{Equ:Possion_equation} can be treated as the Poisson equation, i.e., a large-scale sparse linear system, based on the grid. This linear system involves a large number of free parameters. %During the simulation, we use Marker-and-Cell (MAC) grids to discrete the computation space. 
%%%and use many time steps to iteratively simulate fluid movement.
%fluid simulation without losing numerical accuracy.
%After discretization, each MAC grid stores velocity components $\vec{u}^*$ on the face of the grid, and pressure $\vec{p}$ at the center of the grid. 
%\textcolor{wq}{During the simulation, we use many time steps to divide the simulate fluid movement. At each time step,  we solve the Poisson equation to ensure simulation stability.
%After solving the Poisson equation in each time step, pressure $\vec{p}$ in Equation~\ref{Equ:Possion_equation} is used to update the velocity $\vec{u}$ in Equation~\ref{equ:NS_momentum}.
%The solving process for the Poisson equation is highly computationally intensive and involves large iterative computation to converge to a small residual. This iterative computation can be solved by a traditional numerical method, such as the Preconditioned Conjugate Gradient (PCG) method (line 6 to 12). In this paper, we use a neural network based approximation to solve the Poisson equation and replace the PCG process in Algorithm \ref{Eulerian algorithm}.}

%enabling Bayesian optimization to guide the network morphism for efficient neural architecture search. The framework develops a neural network kernel and a tree-structured acquisition function optimization algorithm to efficiently explores the search space. 
%\textcolor{dong}%because the model with more than one layers deleted frequently violates the user requirements on quality loss (e.g., less than 20\% quality loss), based on our experiments. %\textcolor{red}{($r > \frac{|L|}{2}$ doesn't work well, why choose $r > \frac{|L|}{10}$, not $r > \frac{|L|}{4}$, $r > \frac{|L|}{5}$ or others, do we need some further explanations?)} %After transformation, we have a large number of fast models (128 models). %\textcolor{wq}{We then use Auto-Keras to generate another 128 models that are more accurate as a complement to our fast models. The default morphism operations in Auto-Keras include network widening, network deepening, skip connection, and layer concatenation~\cite{jin2018efficient}.}
%\textcolor{dong}%the x-axis denotes the time cost, and the y-axis is the quality loss. 
%\textcolor{dong}
%For each model, we assume that the quality loss is known by running the simulation. This is a common assumption in some AutoML work~\cite{Sparks:2015:AMS:2806777.2806945, Li:2018:ETM:3187009.3177737}.Adaptive Correlation Filters with

%\textcolor{wq}{\noindent\textbf{Parameter Settings. } As the design space of parameter settings is too large, we need to use a heuristics method instead of exhaust search. (1)Layer pruning. We use a sensitive analysis scheme to estimate the sensitivity of each layer by evaluating the accuracy with pruning whole layers. Experiments show errors of increasing pruned layers grows exponentially. Pruning more than one layer results in large quality violation, i.e, 20\% quality loss.  Note that our basic model is relatively small without too much redundancy. 
%(2)Pooling reduction. We use different pooling rate, i.e., 10\%, 20\% and 30\% of total neurons to study the model sensitivity. Noted that the pooling operation is conducted on all the layers. The pooling rate indicates how many layers are taken into pooling according to the network architecture. Our experiments show that the model accuracy is very sensitive to the pooling rate, so the lowest pooling rate are adopted.   
% (3)Dropout training. We test the efficiency of dropout operation by randomly evaluating four neural network models with different dropout rates, i.e., $5\%$, $10\%$ and $20\%$. As shown in Figure \ref{fig:dropout_loss}, the $10\%$ dropout rate brings better generality and accuracy than the no-dropout. At most time, the $10\%$ dropout rate outperforms the $5\%$ and $20\%$ dropout rate, and is more stable. However, compared to the stable $10\%$ dropout rate, the higher dropout rate, i.e., 20\%, and the lower dropout rate, i.e., 5\%, sometimes generate higher quality loss than the no-dropout models. Hence, we take 10\% as our dropout rate in this paper. 
%As shown in Figure \ref{fig:dropout_loss}, the higher dropout rate generally generates higher quality loss, namely worse results.
%However, compared to the significant quality drop by the $20\%$ dropout rate, the quality by $10\%$ dropout rate obtains comparable results as by $5\%$.
%(4)Dropout models. Although the 10\% dropout rate slightly outperforms the no-dropout models (average 3\% accuracy improvement), only random 18 models (around 15\%) are selected to enrich models diversity due to resource constraints. }

%For each model, we assume that the quality loss is known by running the simulation. This is a common assumption in some AutoML work~\cite{Sparks:2015:AMS:2806777.2806945, Li:2018:ETM:3187009.3177737}.
%After transformation, we have a large number of fast models (128 models). %\textcolor{wq}{We then use Auto-Keras to generate another 128 models that are more accurate as a complement to our fast models. The default morphism operations in Auto-Keras include network widening, network deepening, skip connection, and layer concatenation~\cite{jin2018efficient}.}
%\textcolor{dong}
%enabling Bayesian optimization to guide the network morphism for efficient neural architecture search. The framework develops a neural network kernel and a tree-structured acquisition function optimization algorithm to efficiently explores the search space. 
%\textcolor{dong}
%In Section~\ref{sec:challenge}, our experimental results demonstrate tremendous differences in simulation quality and performance when using various input problems and neural network models. So we develop a quality-aware runtime design to achieve both faster and more accurate simulation simultaneously. In order to achieve this goal, we need a method to evaluate the model being used and switch to a suitable one (if necessary). However, as a representative of evaluating the accuracy of the simulation, the final quality loss cannot be obtained during runtime. %In practical, as the exact solver (PCG method) will not be executed in advance, we are unable to calculate $Q_{loss}$ of output, which needs to compare with ground-truth data. Therefore, it is necessary to propose a quantitative metric to predict $Q_{loss}$ by the objective function of neural networks, i.e., $DivNorm$ claimed in Equation~\ref{Equ:Objective_function}. %Driven by expecting use $DivNorm$ to guide simulation and bound $Q_{loss}$, we try to figure out the relationship between $DivNorm$ and $Q_{loss}$ at each simulation time step. We have multiple observations when using multiple neural networks at runtime: 
%\textcolor{red}{Pending: observations do not support the construction of the metric very well. We need to polish it.}
%\textcolor{xz}{Through theoretical speculation and comparison of a number of experiments as shown in Figure~\ref{fig:sec6_1}, several empirical observations have been proposed.}
%\textcolor{dong} %\item \textbf{Observation 2}: $Q_{loss}$ increases at a high rate at the beginnings and linearly increases at a certain degree; %\item \textbf{Observation 3}: When we switch to the other neural network models in the middle of the simulation, Observation 2 is still valid.%Based on the above observations, we suspect that the cumulative $DivNorm$ may be related to $Q_{loss}$ or has a similar increasing tendency. Then we define the cumulative $DivNorm$ at the $n{\text{-th}}$ time step as follows.

%\textcolor{dong}%The $rp$ is a measurement of the strength of the linear association, and $rs$ is a measurement of the monotonic relationships. 

%\textcolor{red}{Hence it is possible to use the accumulation of $DivNorm$ across time steps to predict the final simulation quality loss $Q_{loss}$ in the last time step.} We define the accumulation of $DivNorm$ after $n$ time steps, $CumDivNorm$, in Equation~\ref{eq:cumdivnorm}.}
 %and also proves the reliability of our speculation.%reveal the relationship between $CumDivNorm$ and $Q_{loss}^{ts}$ by calculating the $rp$ and $rs$ formulas. 
%In our case, $x$ and $y$ are two variables representing $CumDivNorm$ and $Q_{loss}$. Then we use 20480 input problems ($n=20480$ in Equations~\ref{eq:rp} and~\ref{eq:rs}) as $x_i$ and $y_i$ to calculate $rp$ and $rs$. And our calculation shows that $rp=0.67$ and $rs=0.73$. Hence, we conclude that there is a strong correlation between $CumDivNorm$ and $Q_{loss}$. 
%\noindent\textbf{Predicting  \textbf{wq}{Linear regression.}%Based on the strong correlation conclusion, prediction of $Q_{loss}$ involves predicting the value of $CumDivNorm$ in advance. Therefore, it is an unavoidable problem to quickly obtain the value of $CumDivNorm$. 
%\textcolor{dong}{ \emph{CumDivNorm}.}%\textcolor{xz}{In Figure\ref{fig:sec6_1}, $DivNorm$ becomes stable after a few time steps. delete it?} 
%Since $CumDivNorm$ is the cumulative sum of $DivNorm$,
%\textcolor{red}{Check if the following sentence is correct, once Wenqian updates Figure 6.}
%\textcolor{dong} %in a check interval \textcolor{dong}{(the interval is five time steps in our work)}. Those values are used to build a linear regression model, $f_{k}(x) = ax + b$, by the least square method, where $x$ is the time step and $f_{k}(x)$ is the predicted $CumDivNorm$. Note that the values to build the linear regression model must be collected \textit{after} the growth rate becomes stable. In our study, we skip the \textcolor{dong}{first two time steps} to make sure the trend is stable.
 

%The increasing trend of $CumDivNorm$ makes it is possible to predict the value of $CumDivNorm$ at the final step in the middle of the fluid simulation. In particular, we collect the values of $CumDivNorm$ in \textcolor{xz}{a suitable time steps that is used to avoid unstable growth during the warm-up stage,} and then fit the collected values to a linear regression model, $f_{k}(x) = ax + b$, by the least square method, where $x$ is the time step. Then we can predict $CumDivNorm$ at the last time step.Based on the above exploration, the fitting curve can be expressed as:


%\begin{equation}
%   min \sum_{i=1}^{L} \Big(f_{k}(i)-CumDivNorm_{i}\Big)^2,
%   \label{equ:fitting_curve}
%\end{equation}
%where $L$ is time step of check interval for pre-execution phase.
%\algsetup{linenosize=\small}
%\scriptsize %\REQUIRE Input execution records ${S_1,S_2,...,S_N}$.
%\STATE \textbf{Preparing Neural network models:} 
%\STATE 1) Use MLP to choose neural network models;
%\STATE 2) Select some approximate candidates ${M_1,M_2,...,M_K}$ that satisfy user metric. % $U(Q,T)$.%\noindent\textbf{Predicting \emph{Quality Loss}.}%Although the Pearson's and Spearman's correlation coefficient show a strong relationship between the $CumDivNorm$ and $Q_{loss}$, this qualitative analysis is not adequate to give a quantitative prediction for the quality loss $Q_{loss}$ based on a given $CumDivNorm$. To address the above problem, we use a lightweight method to predict the value of $Q_{loss}$ based on the predicted $CumDivNorm$.
%\textcolor{dong}{%\textcolor{xz}{(change to 4? there are too many 5.)}.
%}

%In particular, we use the K-nearest neighbors (KNN) method. In the preparation stage, we first collect a large number of the ($CumDivNorm$-$Q_{loss}$) pairs from several input problems and groups with different models. In the determination phase, the predicted $Q_{loss}$ is calculated based on the average of the k (usually 5) pairs which are closest to the specific $CumDivNorm$ among the current candidate group. %This method does not need to traverse all data pairs, so it does not cause large runtime overhead.
%With the guidance of the \textcolor{xz}{predicted quality loss ($Q_{loss}'$) by KNN method}, we design a quality-aware model-switch algorithm, which can select a neural network model whose $Q_{loss}$ can meet the user requirement on the simulation quality, $q_{u}$. 

%Algorithm~\ref{alg:online_algorithm} depicts the runtime algorithm. Based on the construction of the MLP-based quality controller (Section ~\ref{sec:MLP}), we obtain several promising candidates. Each candidate contains the predicted probability of success and the execution time required in the fluid simulation. We simply use execution time as the indicator to reflect the computation overhead of each candidate.  
%\textcolor{wq}{First, we collect $CumDivNorms$ in the first check interval, calculate the $CumDivNorm^{final}$ using the constructed linear regression model, and predict the $Q_{loss}$ by KNN algorithm. Then, we compare $Q_{loss}'$ with the user requirement $q$. If $Q_{loss}'$ relatively equals to $Q_{loss}$, the current model enable meet the user requirement. The runtime algorithm continues to use the current neural network model. But if $Q_{loss}'$ is much greater or less than $q$, then the runtime algorithm chooses a more accurate model with longer execution time or a more coarse model with faster speed. If all the neural network models cannot meet $q$, we restart the simulation and use the traditional simulation method (i.e., PCG method). The above model switch process happens periodically (the period is named ``check interval''). We calculate $CumDivNorms$ at the end of every check interval to determine if the model switch is necessary.}


%network model with the shorter execution time than the current model and the highest probability among the remaining models. Otherwise, if predicted $Q_{loss}'$ is much lower than demanding $Q_{loss}$, the runtime algorithm selects a more accurate candidate with longer execution time and repeats previous operations until the optimal approximate model is found. If all the neural network models cannot meet the user requirement $q_u$ , then we restart the simulation and use the traditional simulation method (i.e., PCG method).
%(by balancing accuracy and overhead of the pre-execution step of three, five, and 10, and choosing the most suitable one), %and uses five time steps to collect $DivNorm$ for calculating $CumDivNorm$. And the main overhead of finding the best model is pre-execution which could be time-consuming. After a lot of experiments and analysis, our runtime algorithm takes an average of ~5 time steps to find the optimal solution. With the number of time step increases, these overheads are greatly diluted and the proportion of overhead will be decidedly reduced.More detailed discussion will be introduced in Section ~\ref{sec:Analysis_of_Runtime_System}.%In streaming applications~\cite{khudia2015rumba, Krishnan:2016:IDA:2872427.2883026, asplos14:samadi}, it also involves NN-based approximate methods for efficient simulation.Depending on applications, the data can be images, videos, a sequence of words, or a piece of audio, etc. %These approaches train a black-box machine learning system to predict the output produced by an exact solver using neural networks for the Eulerian method. %In this context, having accurate and efficient models for simulating a real-world environment is crucial for developing new learning systems~\cite{Hamrick2016ImaginationBasedDM}.   

%\textcolor{red}{The existing proposed NN-based approximation approaches ~\cite{yang2016data,hong2004precipitation,tompson2017accelerating} lack flexibility with only constructing one neural network model and hard to meet simulation quality for each input problem. Such limitation makes this approach a poor flexibility as it is inaccessible and unusable for some users. Another approach proposed by Ronald Fedkiw et al ~\cite{Fedkiw:2001:VSS:383259.383260} aims to numerical smoke simulation for computer graphics application. However, it can not select the neural network models at run time to enable the best performance, nor extend to general DNNs instead of CNNs. Meanwhile, these proposed approaches can only approximate the fluid simulation with high accuracy for some input problems not for all. Our proposed framework aims to address these limitations in the fluid simulation scenario to some certain extent.}%have become a favorite field in recent years. There are a couple of successful cases. In~\cite{ml_fft}, Smith et al. use a DNN to replace Discrete Fourier Transform (DFT). The Quantum chemistry (QC) simulation obtains 10e4x speedup at a high accuracy. 

%\textcolor{dong}{(2) The pooling rate (Operation 3). Our current method limits the total number of neurons to be replaced to be 10\% of total neurons (i.e., the pooling rate is 10\%). We change the pooling rate to be 5\%, 20\%, and 30\%. Our experiments show that the model accuracy is very sensitive to the pooling rate. Using 20\% and 30\% lead to at least \textcolor{red}{xxxx\%}  quality loss on average. While using 5\% as the pooling rate, the quality loss is close to that of using 10\% (the difference is less than \textcolor{red}{xxxx\%}).}

%\textcolor{red}{Will the dropout rate only impact the training time, not inference time?}
%\textcolor{dong}%Due to resource limitation, we randomly take 8 models for sensitivity study of dropout rate.%and provide a more consistent quality guarantee. 
%Compared to the significant quality loss by the $20\%$ dropout rate, the quality loss by $10\%$ dropout rate obtains competitive accuracy but less neurons (less execution time) by $5\%$. %Our experiments show that the $10\%$ dropout rate brings better model generality and accuracy than without any dropout. For example, the quality loss with 10\% dropout rate is $0.189$, while the non-dropout net obtains $0.209$. %However, compared to the stable $10\%$ dropout rate, the higher dropout rate, i.e., 20\%, sometimes generate higher quality loss than the no-dropout models. While the lower dropout rate, i.e., 5\%, does not introduce sufficient runtime speed-up. Hence, to balance the speedup and accuracy, we take 10\% as our dropout rate in this paper. }

%\textcolor{red}{Give a summary statement here. Using the case of pooling rate as an example.}}
%\textcolor{dong}%\textcolor{wq}{\noindent\textbf{Parameter Settings. } As the design space of parameter settings is too large, we need to use a heuristics method instead of exhaust search. (1)Layer pruning. We use a sensitive analysis scheme to estimate the sensitivity of each layer by evaluating the accuracy with pruning whole layers. Experiments show errors of increasing pruned layers grows exponentially. Pruning more than one layer results in large quality violation, i.e, 20\% quality loss.  Note that our basic model is relatively small without too much redundancy. 
%(2)Pooling reduction. We use different pooling rate, i.e., 10\%, 20\% and 30\% of total neurons to study the model sensitivity. Noted that the pooling operation is conducted on all the layers. The pooling rate indicates how many layers are taken into pooling according to the network architecture. Our experiments show that the model accuracy is very sensitive to the pooling rate, so the lowest pooling rate are adopted.   
% (3)Dropout training. We test the efficiency of dropout operation by randomly evaluating four neural network models with different dropout rates, i.e., $5\%$, $10\%$ and $20\%$. As shown in Figure \ref{fig:dropout_loss}, the $10\%$ dropout rate brings better generality and accuracy than the no-dropout. At most time, the $10\%$ dropout rate outperforms the $5\%$ and $20\%$ dropout rate, and is more stable. However, compared to the stable $10\%$ dropout rate, the higher dropout rate, i.e., 20\%, and the lower dropout rate, i.e., 5\%, sometimes generate higher quality loss than the no-dropout models. Hence, we take 10\% as our dropout rate in this paper. 
%As shown in Figure \ref{fig:dropout_loss}, the higher dropout rate generally generates higher quality loss, namely worse results.
%However, compared to the significant quality drop by the $20\%$ dropout rate, the quality by $10\%$ dropout rate obtains comparable results as by $5\%$.
%(4)Dropout models. Although the 10\% dropout rate slightly outperforms the no-dropout models (average 3\% accuracy improvement), only random 18 models (around 15\%) are selected to enrich models diversity due to resource constraints. }
%In this work, we propose an adaptive neural network-based approximation method to accelerate the Eulerian fluid simulation, which includes three modules (approximation model construction, offline output-quality control, and quality-aware runtime design). Its novelty is gathering a set of model topologies that naturally enables the adoption of a quality-aware runtime algorithm to make full use of the advantages of multiple constructed approximation models and dynamically select the optimal one by predicted $CumDivNorm$. In addition, the proposed approach not only improves the success rate to meet the user requirement on the simulation quality, but also obtains higher performance than Tompson’s method. We hope that our results could inspire more interesting in input-sensitive cases by neural network-based approaches.
%Similar to the previous evaluation results, we use 20,480 input problems. %\textcolor{dong}{%} %it wastes too many time steps to search the optimal model and the accuracy cannot be enhanced by available candidates using the limited remaining time steps.

%figure 9: quality loss(google model VS our framework)%\href{http://mantaflow.com/}
%\textcolor{green}{(Are we sure the readers understand  "evaluation and training dataset" here?)}  %samples
%\textcolor{green}{(Here I don't use the word "samples", because I'd like to put the discussion into the context of fluid simulation.}%\textcolor{blue}{outliers are  whose distance to the lower quartile or upper quartile larger than 3 $\times$ interquartile range. The interquartile range is the distance between lower quartile or upper quartile. let's simplify it and use a reference here.}%In our study, we want to study how the two methods perform with different input problems, in terms of the simulation quality. 
%Second, the usage of neural network models lacks flexibility. During run-time, they use an identical neural network throughout the whole execution, and cannot adjust the neural network model to meet the user requirement. For instance, some specific samples might require accurate model while others are restricted with time consumption. %some case don't need a too accurate model. During neural network model construction, the developer intuitively builds an approximate model with a specific trade-off between performance and accuracy without knowledge of user demands. While one model may not be capable enough to meet all requirements of the different practical environment, e.g., restrict demand of accuracy or performance.%%Third, current neural network models lack sufficient generalization ability to fit diversified fluid samples. %Not only one neural network model disable to meet different user requirements on performance and accuracy, \textcolor{red}{but also it has a quality variation on different inputs}. 
%One single neural network model suffers from a problem that it is hard to cover multiple inputs and provide flexibility for different user demands.
%%Due to the intrinsic nature of neural network based algorithms, the approximate model is a comprehensive model to obtain overall performance but loses its preciseness on some particular samples. This brings an impact of quality violations. Using a single approximate model across multiple inputs either leaves the performance opportunities on the table, large outputs quality violations, or both.

%\textcolor{dong}
%Third, there is no \textit{systematic} approach to construct neural network models for the fluid simulation, and the model construction tends to be heuristic. The neural network can be built with various topologies: we can have a different number of layers, and within each layer, we can have a different number of neurons. How to construct a neural work to meet the requirement of performance and simulation quality of domain scientists is challenging. Currently, domain scientists build a neural network by changing an existing one intuitively. There is no systematic approach to help them build neural networks for HPC applications. The recent work on Auto-Keras~\cite{jin2018efficient} and AutoML~\cite{escalante2019automl} aims to automatically generate a neural network model with the best accuracy. However, they lack concerns on high performance (execution time), and they focus on image processing or natural language processing. Hence, they are not directly usable for HPC.

%First, the used neural network models are constructed in a highly intuitive way. Neural network architectures and hyper-parameter settings are empirically trained and optimized to improve the performance of neural networks. The field experts may not able to master a \textit{systematic} way to explore neural network models to satisfy their performance and accuracy requirements. Some users with limited machine learning expertise may expect Auto-Keras~\cite{jin2018efficient} or AutoML to generate a neural network model. However, those tools usually generate one single high-quality models with high computation overhead. Also,  those tools are typically designed for image processing or natural language processing and are not directly usable for HPC.
%(or %how many of them can outputs can achieve users' requirements among all input problems.
%\textcolor{green}{(what is the success rate? We define it in the evaluation section, not here)}
%%%fit the transformation from input to output.
%capture the multi-modal distribution of numerous inputs.\textcolor{green}{what is the multi-modal distribution?} \textit{samples} in the language of machine learning). %during the training phase of the neural network models which are conducted off-line and have no runtime overhead. %First, we take out neural network models \{$M_1, M_2,..., M_K$\} from the 14 neural network models. For each neural network model $M_k \in \{M_1, M_2,..., M_K\}$, we get $N$ execution information by $N$ input problems ($N=20,480$ input problems in this paper). Given a $M_k$, the execution information $S_n^k \ \in \{S_1^k, S_2^k,..., S_N^k\}$ includes the simulation quality loss $q_n^k$ and time cost $t_n^k$. 

%\noindent\textbf{Positive and Negative Sample Generation.}%Based on $EI_n^k$, $q_n$ and $t_n$, we can easily label the sample as success (i.e., meeting both requirements on quality and execution time) or not success. We use $r_{n,k}$ to represent the label, and the values of 1 and 0 of $r_{n,k}$ represent success and not success of meeting the user requirements respectively.}

%Then, when execution information $S_n^k$ for $M_k$ is ready, we decisively construct a positive training sample and a negative training sample. In particular, we define a positive quality requirement $q_n^{pos}$ as whose quality loss requirement looser than the measured quality loss $q_n$, i.e., $q_n^{pos}(>q_n)$.%, based on a execution result $s_n$. Similarly, a positive time requirement $t_n^{pos}$ is defined as whose time limitation is longer than measured execution time $t_n$, i.e., $t_n^{pos}(> t_n)$. 

%We construct positive training samples which must meet the requirements of quality and time at the same time. Otherwise, a training sample in whose quality requirement is negative, $q_n^{neg}(<q_n)$, or the time requirement is negative, $t_n^{neg}(< t_n)$, will be defined as a negative training sample. 
%so that the high-level semantic information can be extracted from low-level features.
%\textcolor{red}{Consider to re-phrase the above sentence to make it clearer. What is "high-level semantic"?}
%The used MLP requires an input layer with 48 nodes. We use 6 hidden layers to extract the high-level features of the input information. The node numbers of these hidden layers are 32, 32, 16, 16, 8 and 8 respectively. All the hidden nodes are activated with ReLU units to increase the non-linearity of the model. The output layer with a single node is activated with a sigmoid function. The network architecture is depicted in Figure~\ref{fig:MLP_model}.




%\textcolor{wq}{During the MLP construction, we try to figure out the most effective and efficient model architecture. When composing the MLP model, we follow the rule that in a topology of neural network, a deeper layer generally has less neurons than a shallower ones (neurons gradually decrease), so that the high-level semantic information can be extracted from low-level features.
%so as to make the final prediction for the success rate. The same rule can be found in many discriminative neural networks such as Alex-Net\cite{krizhevsky2012imagenet},  VGG-Net\cite{simonyan2014very}, etc. We develop 5 MLP models in total with the changes on the depth of hidden layers. The architectures of these models are briefly described as follows: 
%\begin{itemize}
%    \item $MLP_1$ has 4 layers with 48, 32, 16, 1 neurons;
%    \item $MLP_2$ has 5 layers with 48, 32, 16, 8, 1 neurons;
%    \item $MLP_3$ has 6 layers with 48, 32, 32, 16, 8, 1 neurons;
%    \item $MLP_4$ has 7 layers with 48, 64, 32, 32, 16, 8, 1 neurons;
%    \item $MLP_5$ has 8 layers with 48, 64, 64, 32, 32, 16, 8, 1 neurons.
%\end{itemize}
%As shown in Figure ~\ref{fig:mlp_loss}, we present the training loss of 5 MLPs. We can find that the convergence speeds and final losses of $MLP_3$, $MLP_4$, $MLP_5$ are faster than those of $MLP_1$ and $MLP_2$. Compared with the $MLP_3$ model, $MLP_4$ or $MLP_5$ does not achieve significant advantage although deeper layers are adopted. The $MLP_3$ exhibits a balanced trade-off between the prediction accuracy and the model size, and is thus chosen as our default model in this paper.}
%By calculating the expected time cost of each $M_{k}$ model, we remove some models from the model pool that are larger $T_{total}$ than user time constraint $t_u$. We collect these remaining models as \textit{approximation candidates} for runtime algorithm (as we will discuss in Section \ref{Quality-Aware Model-Switch Algorithm}).}
 
%where $T'$ is the execution time . By calculating the expected time cost of each $M_{k}$ model, we remove some models from the model pool that are larger $T_{total}$ than user time constraint $t_u$. We collect these remaining models as \textit{approximation candidates} for runtime algorithm (as we will discuss in Section \ref{Quality-Aware Model-Switch Algorithm}).%In the pre-screening stage, when the users give specific requirements on simulation quality and time cost, we can use the trained MLP to give an estimation $\hat{r}_{n,k}$, which represents the effectiveness of a neural network model, and exclude some unsuitable models in advance. A larger value of $\hat{r}_{n,k}$ represents a higher success rate. In other words, a neural network model with a high success rate can achieve both time and quality requirements on most input problems. We try to filter out neural network models which can bring performance (execution time) benefits on given success rate, and use the most accurate model in \textit{Neural Network Models} instead when the selected neural network model fails.
%%%We use the binary cross-entropy loss function to evaluate the distance between $\hat{r}_{k,q,t}$ and $r_{k,q,t}$, shown in Equation~\ref{eq:mlp_loss_func} (we omit the subscript ${n,k}$ for simplicity). 
%By minimizing the loss between the estimation $\hat{r}_{n,k}$ (a float point number) and the ground truth label $r_{n,k}$, the trainable parameters of MLP can be optimized to fit the whole dataset. We use the binary cross-entropy loss function to evaluate the distance between the estimated success rate $\hat{r}_{n,k}$ and ground-truth label $r_{n,k}$. The loss function is described as follows:
%\begin{equation}
%\label{eq:mlp_loss_func}
%    loss(\hat{r}, r) =  \sum_{n, k} \Big[ r * log(\hat{r}) + (1 - {r}) * log(1 - \hat{r})\Big],
%\end{equation}
%where we omit the subscript ${n,k}$ for simplicity.
%For a positive training sample, we use a binary number $r^{pos}_{n,k} = 1$ to label the result as a success. The input feature of a positive training sample, shown in \textcolor{dong}{Equation~\ref{eq:input_feature_positive_sample}},  consists of the positive quality requirement $q_n^{pos}$, the positive time requirement $t_n^{pos}$ and the hyper-parameters of the training neural network model.%\textcolor{dong}{In Equation~\ref{eq:input_feature_positive_sample}, $l_k$, $\overrightarrow{ker}_k$, $\overrightarrow{chn}_k$, $\overrightarrow{pool}_k$, $\overrightarrow{unp}_k$, and $\overrightarrow{res}_k$ are hyper-parameters, representing, the number of layers, the kernel sizes,  channel number,  pooling size, unpooling size,  and residual connection of each layer respectively.
%The largest number of layers is no more than 9.
%Each of the last five hyper-parameters is a vector  composed of nine components that indicate properties of each layer. Therefore, the total length of the above input feature vector is $F^{pos}_{n,k}$ is $3+5*9 = 48$.}

%\textcolor{dong}{For a negative sample, the input feature is formulated similarly (shown in Equation~\ref{eq:input_feature_negative_sample}), and its label is $r^{pos}_{n,k} = 0$.} 
%On the other side, the negative sample is labeled by $r^{neg}_{n,k} = 0$ as failures, whereas its feature is composed as follows:
%\begin{equation}
%\label{eq:input_feature_negative_sample}
%F^{neg}_{n,k} = \Big(q_n^{neg}, t_n^{neg}, l_k,  \overrightarrow{ker}_k, \overrightarrow{chn}_k, \overrightarrow{pool}_k, \overrightarrow{unp}_k, \overrightarrow{res}_k\Big)
%\end{equation}

%This paper tackles these problems and design a run-time adaptive algorithm to provide dynamic choices. In this paper, we aim to provide efficient approximate models for different user requirements, from computational fluid simulation to computer animation. Moreover, we expect each input can achieve relatively stable quality during simulation. Under such circumstances, we face some challenges during our system design.%and the model generation must be automatic. %How to explore and exploit efficient neural networks? The need for significant improvement of processing throughput for fluid simulation expects efficient neural networks for approximate computing, where small amounts of output accuracy can be traded for relatively large improvements in performance improvement or energy saving. How to yield the right trade-off between performance and accuracy facing different user demands. During the model construction, developers intuitively build a neural network based on their machine learning training experience. While, as approximate computation, users may expect a fixed neural network to achieve either a high-quality target, high energy saving, or a specific trade-off.%How to build the calibration computes both exact and approximate results at run-time. Calibration at run-time computes both exact and approximate results, then compare them to measure the accuracy of the approximate approaches to guide simulation. In practical, fluid simulation won't run exact approaches to validate the accuracy of the approximate models. There leaves a question that how to use the loss of approximate models guide the run-time simulation and achieve the final output quality target.%Focusing on the worst case accuracy can result in overly conservative approximation for other input, while compromising on the average case accuracy may fail to deliver sufficient accuracy in the worst case.
%Focusing on the worst case accuracy can result in overly conservative approximation for other input, while focusing on average case accuracy may be overly aggressive and fail to deliver sufficient accuracy in the worst case.
%How to select appropriate approximate models for different samples. It is hard to use one approximate model to cover multiple inputs. %In this paper, we propose a self-tuning approximation for fluid dynamic simulation and provide quality control during run-time by a quality-aware monitor. Roughly speaking, given a permissible error by users, a set of most promising approximate models are filtered out from neural network pools to accelerate fluid simulation. Then, these approximate models are adaptively chosen by different inputs during runtime to exploit both the power of acceleration and accuracy guarantee under a run-time quality aware monitor. Our framework proposed effective methodologies for existing problems but leave the following challenges.%The main contributions of this work are as follows:
%\begin{itemize}
%\item We generate effective and efficient neural network approximation candidates based on a basic model, screen and gather them as a comprehensive approximate model pool. 
%\item We build an MLP(Multilayer Perceptrons) model to guide approximate candidates choice under user demands.  The MLP model not only filters out the suitable approximate models for user demands but also provide a dynamism search space for different input samples.
%\item We profile and collect the stat of error propagation during the fluid dynamic simulation. Analyze the characteristics of error propagation and build a model to bound relative error of certain frames to avoid error overflow and achieve our final quality target. 
%\item We adaptively switch approximate models during simulation to get the most appropriate approximate model for each sample. The approximate model can be self-tuned to vary the fidelity of produced output.
%\end{itemize}


\begin{comment}
\begin{algorithm}[!t]
%\algsetup{linenosize=\small}
%\scriptsize 
\small
\caption{The quality-aware model-switch algorithm}
\label{alg:online_algorithm}
\begin{algorithmic}[1]
\REQUIRE User metric $U(q, t)$.
\REQUIRE Input sample set ${S_1,S_2,...,S_N}$.
\STATE \textbf{Approximate candidates (neural network models) preparation:} 
\STATE 1) Use MLP to choose neural network models;
\STATE 2) Select some approximate candidates ${M_1,M_2,...,M_K}$ that satisfy user metric. % $U(Q,T)$.
\FOR{$S_n \in {S_1,S_2,...,S_N}$}
\STATE \textbf{Pre-execution:}
\STATE Choose the candidate $M_k$ with the highest successful rate. 
\REPEAT
\STATE Forward $M_k$ for $L$ time steps ($L$ is time step of \textcolor{xz}{pre-execution})
\STATE \textbf{Prediction of quality loss:}
\STATE 1) Fit the curve of $CumDivNorm$ with respect to the time step;
\STATE 2) Predict the $CumDivNorm'$ of the final time step $t=N$ by linear regression;
\STATE 3) Predict the $Q_{loss}'$ of the current approximate candidate by KNN method; 
\STATE  \textbf{Model Switch:}
\IF{$Q_{loss}'$ is satisfied $q_u$}
\STATE Continue using the current candidate; 
\ELSIF{$Q_{loss}'$ much less than $q_u$ }
\STATE Switch to a faster candidate;
\ELSIF{$Q_{loss}'$ can't satisfied $q_u$}
\STATE Switch to a more accurate candidate;
\ELSE
\STATE Restart by PCG method;
\ENDIF
\STATE $t \gets t+L$ ; 
\UNTIL reach to the final time step $n$
\ENDFOR
\end{algorithmic}
\end{algorithm}
%\vspace{-10pt}
\end{comment}


\begin{comment}
%
In our simulation, we currently don't take fluid viscosity into account and drop the viscosity term from equation \ref{equ:NS_momentum}.
%
The equation is rephrased as 
\begin{equation}
\label{equ:Euler_equation}
    \frac{\partial \vec{u}}{\partial t} =  - \vec{u}  \cdot \bigtriangledown \vec{u} - \frac{1}{\rho} \bigtriangledown p + \vec{f}  
\end{equation}
and called \textit{Euler Equation}.
%
For incompressible fluid, a vector field has to satisfied the Equation \ref{equ:Euler_condition}, named ``divergence-free''.
%%
To solve these two Equations \ref{equ:Euler_equation} and \ref{equ:Euler_condition}, we use standard operator spitting method to split into three parts, i.e., advention step, external force step, and pressure projection step.
%
The basic Eulerian procedure is shown in Algorithm \ref{Eulerian algorithm}.
%
This condition is enforced by adjusting the pressure field at each integration step. 
%
Additionally, we use a semi-Lagrangian method \cite{stam1999stable} to advect field value instead of using the advection term directly to ensure the simulation stability. 
\begin{algorithm}
\caption{The Fluid Simulation Process}
\label{Eulerian algorithm}
\begin{algorithmic}[1]
\REQUIRE Simulation time step $N$; 
\STATE Start with an initial divergence-free velocity field $\vec{u}^0$
        \FOR{ $n \gets 1$ to $N$ }        
        \STATE Advection: Set $\vec{u}^{A}$ = advect($\vec{u}^{A}$, $\Delta t$, $q$)\\
%\State Advection: Set $\vec{u}^A$ = advect($\vec{u}^A$, $\Delta t$, $q$) \\
\STATE Add body force $\vec{u}^B = \vec{u}^A +\bigtriangleup t \vec{f}$ \\
\STATE Solve Equation: $\vec{u}^{n+1} = \vec{u}^{B} - \Delta t \frac{1}{\rho} \Lambda \vec{p}$
%\State Solve Equation: $\vec{u}^{n+1} = \vec{u}^B - \Delta t \frac{1}{\rho} \Lambda \vec{p}$ \\
\STATE Pressure Projection: Set $\vec{u}^{n+1}$ = project($\bigtriangleup t$, $\vec{u}^B$)
\ENDFOR
\RETURN{0}
\end{algorithmic}
\end{algorithm}
\end{comment}
%
%This formula is consisted by advection part, viscosity part, pressure part and body force part.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textcolor{blue}{para 2: how these equation are applied in grid based simulation}
%\textcolor{blue}{In this paper, we focus on fluid simulation without considering fluid viscosity (i.e., the Eulerian fluid simulation).}
%take fluid viscosity into account, and only consider fluid with zero viscosity.

%To ensure the simulation stability, i.e., a constant density, Equation ~\ref{equ:Euler_condition} is enforced to be solved by adjusting the pressure field at each integration time step and can be transformed as 

\begin{comment}
We design a run-time adaptive algorithm to dynamically adjust available models to achieve target accuracy at low time cost.
Our novelty of model selection during the simulation are as follows. \textcolor{green}{Should the novelties of model selection correspond to the next three subsection?}
\begin{enumerate}
    \item We dynamically switch the model using execution time instead of time steps. \textcolor{green}{What is the difference between execution time and time steps?}
    \item We use checkpoints to guarantee the quality benefits.\textcolor{green}{checkpoint frequency?}
    \item We develop an adaptive run-time algorithm to guarantee the execution benefits.
\end{enumerate}
%
{\color{blue} 3 pages explain how does the predictor work?}

add a discussion on the requirement of our runtime algorithm. (1) The algorithm needs to have a metric that allows us to quickly evaluate the output quality; (2) We need to be able to predict the final output quality at any moment of the CFD simulation. 

%\textcolor{green}{
\textcolor{red}{the motivation of this paper, the gap of quality loss based on different samples are very large.see background 2.3 and the figure 1. discuss about the flaw.
Third, how to construct neural network models covering sufficiently large number of input problems and ensuring overall performance benefit is a challenge. 
Focusing on the worst case accuracy can result in overly conservative approximation for other input, while compromising on the average case accuracy may be fail to deliver sufficient accuracy in the worst case.}

Comparing with previous experimental results(\textcolor{red}{where is the results? form sec4??}), it is obvious that various CNN-based approximate models can bring huge benefits in performance and accuracy under suitable conditions.\textcolor{red}{we need also explain the quality variation here so we need use multiple neural networks} 
In order to make full use of the advantages of approximate models, we designed a Quality-aware Runtime System (Smart-fluid) to achieve both faster and more accurate simulations by automatically selecting the optimal CNN-based approximate model at each check point of solution. 
However, since CNN-based approximate models can only acquire execution time and model loss at current time steps in fluid simulation, the final output quality of this model can not be obtained directly before all iterations are completed. 
Therefore, it is necessary to propose a quantitative metric and method, which could predict the output quality by measured DivNorm at any stage of CFD simulation. 
\textcolor{red}{From this point of view, we have studied a large amount of experimental data to explore the potential connection between CumDivNorm(Section 6.1), quality loss and output quality(Section 6.2). 
Next, we will introduce the relationship between three parameters and quality-aware runtime algorithm(Section 6.3) respectively.}

\end{comment}

\textcolor{red}{DivNorm: the approximate model loss;
CumDivNorm: sum of DivNorm;
Quality loss: the simulation loss;
background 1 last 2 paras;
explain their relationship
DivNorm: we can know during the runtime;
Quality loss: the simulation loss
challenge: we can't know the quality loss during runtime.
dig their relationship use Spearman's rank correlation.
explain we use the Spearman's rank correlation to quantify the relationship}
In this section, we define two quality-based parameters: 1) \textit{CumDivNorm}, \textcolor{red}{too complicated use a equation to express} which measures the squared L-2 norm of the divergence of predicted velocity as DivNorm at the current time step and accumulates with measured DivNorms in the previous time steps. 2) Quality loss\textcolor{red}{has beed defined in background section \ref{eq:Quality_Metric}}, which evaluates accuracy of approximation by calculating the density matrix of fluid grid and measuring the distance from exact ground truth data. It is noteworthy that the training objective and error propagation of neural network are mainly based on minimizing the second parameter\textcolor{red}{the first parameter}.


Where $\vec{u_t}$ is the predicted density matrix and $\vec{g\_t}$ represents the ground truth data by exact approach.



%Since exact solution or $\vec{g\_t}$ data can not be obtained, then quality loss that depends on exact solution can not be calculated directly either, which makes it impossible to evaluate predicted divergence of current CNN model. 
Since user won't calculate the exact solution $\vec{g\_t}$ data in practical, we can't get quality loss at runtime to guide our simulation.
Therefore, a method of avoiding data dependence of $\vec{g\_t}$ and indirectly predicting quality loss through a designed metric is expect. 
According to our observations, as the number of iteration step increases, the approximate model loss, i.e., the CumDivNorm gradually increases. 
Meanwhile, with more equations are solved, the $\vec{u_t}$ keeps close to the target $\vec{g\_t}$ data and it makes quality loss smaller. 
So we empirically assume that there may be an inverse relationship between these two parameters.\textcolor{red}{explain we use the Spearman's rank correlation to quantify the relationship}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/sec6_1.pdf}
       \vspace{-5pt}
        \caption{.\textcolor{red}{wq:delete?? no use at all}} 
  \vspace{-5pt}
  \label{fig:relationship between CumDivNorm and Quality loss}
\end{figure}



\begin{figure}[t]
  
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/sec6_2.pdf}
       \vspace{-5pt}
        \caption{Network architecture of the proposed MLP model.} 
  \vspace{-5pt}
  \label{fig:a small model}
\end{figure}




To illustrate this idea, we explore possible correlation by a large number of experimental data on multiple samples and CNN models. 
As shown in Figure 6.1, the x-axis represents measured divergence of DivNorm in different scenarios, and the y-axis represents the calculated quality loss. 
By using linear fitting function, the solid line corresponds to a best-fit straight line through these all points, and almost all points are distributed around the solid line. 
More specifically, we use the widely used statistical method (Spearman's Rank Correlation Coefficient) to analysis and prove the relationship between the two parameters. 
Correlation coefficient of all collected scatter points is 0.X, which unanimously shows very high correlation and leads to the same conclusion. 
Therefore, it is possible to predict quality loss with CumDivNorm, and breaks through the bottleneck that cannot be directly evaluated.

As the convergence quality of CNN models does not change much in each iteration step, then the smooth convergence results in slight change for DivNorm and linear growth trend for CumDivNorm. 
As shown in Figure 6.2, x-axis represents time step and y-axis represents CumDivNorm, lines of different colors show multi convergence results by various CNN models and exhibit distinct linear characteristics.
Therefore, in order to minimize overhead and predict quality loss of CNN model in advance, the divergence expectation of CumDivNorm at each time step can be predicted by fitting a straight line with pre-execute for small number of iterations steps.
Based on these observations, we collect the divergence velocity of CumDivNorm in several steps (usually 5 steps) by actual measurement of CNN model, and use the least square method to fit a straight line, thus the expectations of DivNorm at any time step can be predicted, especially for the final performance expectation.


\begin{figure}[h]
  \centering
  \includegraphics[width=45mm]{Figures/image_loss.pdf}
  \caption{Quality Loss.}
  \label{Quality_loss}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=45mm]{Figures/DivNorm.pdf}.
  \caption{DivNorm.}
  \label{DivNorm}
\end{figure}
%

\begin{figure}[h]
  \centering
  \includegraphics[width=45mm]{Figures/cum_sum_Divnorm.pdf}
  \caption{Cumulative Sum of DivNorm.}
  \label{Cumulative_Sum_DivNorm}
\end{figure}
\textcolor{blue}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{WQ:}
\textcolor{blue}{para1:what is DivNorm?}\textcolor{green}{and Simulation quality?}

\textcolor{green}{para2:1)How to find the the connection between DivNorm and Simulation quality?\\
2)By accumulating DivNorm? What is the reason? or pure experimental observation？}

\textcolor{blue}{para2:list the variation of simulation quality loss and DivNorm during the CFD simulation.we try to get a connection between simulation quality loss and DivNorm through cumulative sum of DivNorm. explain the similar tendency of DivNorm simulation quality loss.}





%\subsection{Determination of Output Quality Metric}
%\subsection{Determination of Output quality by predicted Simulation quality}(revised)
\subsection{Output Quality Prediction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Characterization of Divergence Curve}
\textcolor{blue}{Dong: WQ, add some figures to show two points, (1) There is a jumpup phase follow ing by a going-down phase; (2) No matter when we reach a specific accuracy, the divergence curve for a model will behave similar.}
\textcolor{blue}{Dong: WQ, add a pseudo code to show the algorithm}.
\textbf{An example.}
\textcolor{blue}{Dong: WQ, add an example case.}
In general cases, given a fixed quality budget, there is currently no way to guaranteeing a pre-fixed tolerance with respect to the final quality for various inputs.

the schedule of the pipeline(overlapping).


the search methods: the first prediction and the following predictions.

how to implement the overlapping of execution time and prediction time.


where is the checkpoints and how to save useful info (other routes)?

show some result of average running time, the success rate (final outputs achieve expected outcomes) and the overhead of redo previous steps  (how frequent and how long)
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{A Lightweight Model-Switch Algorithm}

With respect to the fact that output quality of CNN model can be predicted by measured DivNorm, then we design a quality-aware model-switch algorithm, which specializes a transparent solver and focuses on solving equations at the fastest speed while ensuring the solution of the goal, and choosing the most suitable model with the change of equations in simulation process. Application developers do not need to care about the choice among the CNN models, but prepare the input sample and user's requirements. Figure 2 shows the execution process of the runtime system, and a specific case is used to instantiate the strategies and algorithms involved in this method.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/sec6_3.pdf}
       \vspace{-10pt}
        \caption{Network architecture of the proposed MLP model.} 
  \vspace{-5pt}
  \label{fig:a small model}
\end{figure}


Typically this runtime system consists of four distinct steps: Step1, model candidate, in which the MLP model predicts the probabilities of various CNN models based on input sample and the top k (usually 5) probabilities are selected. Each model candidate contains predicted probability and the flops required for approximate computation, and flops is also proportional to execution time and solution accuracy. As shown in this example in Figure 6, the highest probability, such as M1, is selected as the pre-executed model; Step 2, model execution is to run the recommended model and collect the CumDivNorms of five iteration; Step 3, fitting and prediction, in which the collected divergence data are used to fit CumDivNorm curve by least squares method, and the output quality is predicted by Spearman's Rank Correlation Coefficient using expectation of CumDivNorm at the end of simulation; Step 4, Model Switch, then we compare predicted output quality with user's requirements, if requirements are met, the current model continue to be used until equation is solved. If it is less than user's requirements, then runtime system select the one that is higher than flops of the current model with the highest probability, and skip to the Step 2. In addition, if all models are unable to meet user's requirements, we restart the calculation and solve this equation by exact method. As shown in the current example, since predicted output quality of M1 model cannot meet user's requirements, then the M2 model is reselected and the Step2 and Step3 are performed, and equation is finally solved using M2 model that meets requirements. The detailed algorithm of the runtime system is shown in Algorithm 1.

A major premise for the runtime system is a set of appropriate models that is used to build a quality-aware model-switch system. The interface of runtime system is mainly composed of two parts based on Inspector-Executor method. The inspector briefly pre-executes model, predicts the output quality that the model can achieve, and choose the fastest and most accurate model that meets the requirements. The executor solves the entire equation by reusing predicted result. say something about accuracy and overhead of runtime system.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%
Based on the prior profiling results, we design an adaptive algorithm to finish the simulation in one time with the success confident $S$(need re-phrase).
%
During the simulation, we calculate the quality based on Equation~(\ref{eq:Quality_Metric}).
%
While, Equation~(\ref{eq:Quality_Metric}) focusing on average case accuracy may be overly aggressive and fail to estimate sufficient accuracy in some worse cases.
% 
As shown in Fig \ref{Model Quality}, even all candidate models quality based on average samples are over expect $Q_{target}$, some samples still deliver over-estimation about their quality.
%
Our design have to supervise the accuracy hindered by input differences and adaptively select models to guarantee the final quality. 

\begin{figure}[t]
  
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/Sec6_2.pdf}
       \vspace{-5pt}
        \caption{Network architecture of the proposed MLP model.} 
  \vspace{-5pt}
  \label{fig:a small model}
\end{figure}


%
During run-time, we use checkpoint to guarantee the quality benefits to prevent redo the whole simulation.
% 
According to the profiling results, we derive a check frequency for the follow-up running time(Need to design a function connecting success rate and check frequency. $check\_freq = f(1/suc\_rate)$).
%
We select an initial model that has the most approximate success rate as the user's setting(a figure needed here).
%
If the success rate is assumed to be high, then the check frequency will be low, meaning that a large check interval is adopted.
The final quality can be developed using Equation~(\ref{eq:Quality_Metric}).
\textcolor{blue}{pending: switch frequency??}



During execution, the total time cost can be expressed as follows,
\begin{equation}
    T_{total} = \sum_{i =1 }^{N} T_{M_{i}} + T_{CKP} + T_{Redo},
\end{equation}
where $T_{M_{i}}$ is the model forward at time step $i$, $T_{CKP}$ is the total checkpoint time cost, and $T_{Redo}$ the total Redo time during the simulation. 

%a Greedy Algorithm after each checkpoint.
%
When doing checkpoint, we record the elapsed time and the left available time. 
%
The model candidates are filtered out of model pool, which satisfy both the quality requirement and time cost limitations for the rest to-be-simulated time steps.
%

We select the best 
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%both the quality requirement and time cost limitations with given success rate.
%
%
%Moreover, the success rate will guide the whole simulation in run-time.
%Based on these model candidates, we do a prior-profiling to examine the success rate of different models that can achieve specified target within one time simulation. 
%
%The success rate of a model is determined by the ratio of successful samples of the test set.
%
%The profiling result is calculated based on the performance statistics during model training phase which is conducted off-line.
%

%By feeding the test samples $s_i (i \in [1, N])$ to a given model $M_k$, we are able to obtain the simulation quality $q_i$ and consumed time $t_i$. 
%So that when users provide their quality and time constraints, we can quickly label each sample $s_i$ with a binary number, i.e., $0$ for a failure case and $1$ for a success case.
%calculate a success rate of model $M_k$ by using the MLP network.
%By forwarding the multiple test samples $s_i (i \in [1, N])$ on a given model $m_j$, we are able to obtain the simulated image quality $q_i$ and consumed time $t_i$. 

%
%Namely, the model $M_k$ is able to process the sample $s_i$ with quality constraints $q_i^{pos} (< q_i) $ and time cost $t_i^{pos} (> t_i)$.
 
%simulation results $r_i$.
%
%On the other side, the model $m_j$ is unable to process the sample $s_i$ at a higher image quality $q^{neg}_i (> q_i) $ or smaller time cost $t^{neg}_i (< t_i)$.

%to design a multi-layer perceptron (MLP) neural network which help the prior profiling, i.e., calculating the success rate through model characteristics under users' demands.
%
%Namely, the model $m_j$ is able to process the sample $s_i$ at $100\%$ success rate. 
%
%We refer to this simulation instance as a successful sample and use a binary number $r_i = 1$ to label the result as a success. 
%simulation results $r_i$.

%the MLP can be trained on these positive and negative instances to extract the useful clues for checking the successful rate of model $m_j$.
%
%The network architecture of the used MLP model is described in the following subsection.
%For each model $m_j (j\in(1,M)$, we can repeat the above process to obtain a corresponding MLP$_j$ for profiling its success rate.
%To satisfy the requirements for users, we insert checkpoints during run-time to guarantee the quality benefits.%If the inferred success rate of all models of our model pool is lower than the given constraint, we will argue users to adjust the metrics $M(Q,T,S)$ until at least one model can satisfy their requirements.
%2.how to train the MLP model to guarantee there will leave some time to redo some failure cases.

%
%
%These model candidates 
%We design a score function to guide the selection of model candidates, 
%\begin{equation}
%    S(M_i) = \alpha Q_{M_i} + \beta T_{M_i}, 
%\end{equation}
%where the coefficient $\alpha$ and $\beta$ are to balance the contributions of quality and time factors.
%
%And they are set to 0.1 and 0.001 empircally. (\textcolor{blue}{Wenqian: Empirical Setting?})

%The predict $CumDivNorm$ can be expressed as follows,
%\begin{equation}
%\label{eq:Quality_Metric}
%CumDivNorm^{'}=f_{k}(n).
%\end{equation}
%
%Where $n$ is the final timestep of fluid simulation.
%
%
%As the program behavior can be change at runtime, Smart-fluid monitors the accuracy and performance dynamically.
%
%At each calibration interval, the quality-aware model switch algorithm check output quality by the related predict $CumDivNorm$.
%%\textcolor{red}{how to calculate the exponentially decay weights in detail by historical data? There are some descriptions in the next sentence, but it is difficult for readers to understand the entire calculation process.}

\begin{comment}
In this paper, we propose to measure the acceptability of the final quality loss using the maximum a \textit{posteriori} estimation.

In this paper, the K-nearest neighbors (KNN) method has been introduced
to predict final quality loss, and high success rates

%
The posterior distribution will be $p(x)$, where $x$ is the predicted $CumDivNorm$.
%
The value of $p(x)$ represents the confidence that the predicted $CumDivNorm$ satisfies the hypothesis.
%
In this case, the hypothesis is that the output quality is better than the user requirement.
%
For example, for a user quality requirement is $0.01$, the confidence of a $CumDivNorm$ value $450$ equals to 93\%.
%
At runtime, we dynamically select the optimal approximate models until the confidence of predict $CumDivNorm$ reach our target.
%
The default confident target is 95\% in this paper. 

\textbf{Efficiency of Loss Prediction.}
use some results to show the accuracy of using $CumDivNorm$ to guide our runtime algorithm. 

\end{comment}

\begin{comment}
\begin{figure}[h]
  \centering
  \includegraphics[width=75mm]{Figures/sample_quadrant.pdf}
  \caption{Sample Quadrant.}
  \label{Sample_quadrant}
\end{figure}
\end{comment}
%
%Therefore, there leaves a question that how to use the measured loss of approximate models (claimed in Equation~\ref{Equ:Objective_function}) to guide the runtime simulation and achieve the final output quality target.


\begin{comment}
\textcolor{blue}{wq, 1-2 paras: how to chose efficient model candidates. 
multi-bandit algorithm, two baseline: light-weighted or accurate; reference: paper SLAQ}

\end{comment}

%This section provides a detailed description of how a MLP-based quality controller chooses and leverages approximate model candidates that are customized and effective for different user requirements.%, and only some special approximate models can meet the limit requirements
%In this section, we design an MLP-based quality controller, which chooses and leverages approximate model candidates that are customized and effective for different user requirements.

%Note that we collect these profiling results during the approximate model testing phase when $M_k$ is well trained.
%As shown in Figure~\ref{Sample_quadrant}, 
 %A whole positive training sample of MLP is consists of  $N\times K$ training samples based on $N$ profiling results on each $M_k \in \{M_1, M_2,..., M_K\}$. 
%All positive training samples are collected as a positive set $I^{pos}$.On the other side, the negative training sample set of MLP i.e., $I^{neg}$, is a collection of training samples that have negative quality i.e., $q_i^{pos}$, smaller time cost $t^{neg}_i$ or both. 
%\begin{equation}
%\begin{split}
 %   &I^{pos} = \Big\{(F_i,r^{pos}) | \\
  %  &F_i = (q_n^{pos}, t_n^{pos}, lay_k,  \overrightarrow{ker}_k, \overrightarrow{chn}_k, \overrightarrow{pool}_k, \overrightarrow{unp}_k, \overrightarrow{res}_k), \\
   % &\forall (n,k) \in [1,N]\times[1,K]\ and\  i\coloneqq n*K+k \Big\}.
%\end{split}
%\end{equation}
%
%We refer these input samples as negative and use $r^{neg} = 0$ to label them as failures.
%All the negative samples form a negative set, 
%\begin{equation}
%\begin{split}
%&I^{neg}=\Big\{(F_i,r^{neg}) |\\
%& F_i= (q^{neg}_n, t^{pos}_n, lay_k,  \overrightarrow{ker}_k, \overrightarrow{chn}_k, \overrightarrow{pool}_k, \overrightarrow{unp}_k, \overrightarrow{res}_k) \ or \ \\
%& F_i=(q^{pos}_n, t^{neg}_n, lay_k,  \overrightarrow{ker}_k, \overrightarrow{chn}_k, \overrightarrow{pool}_k, \overrightarrow{unp}_k, \overrightarrow{res}_k) \ or \ \\
%& F_i=(q^{neg}_n, t^{neg}_n, lay_k,  \overrightarrow{ker}_k, \overrightarrow{chn}_k, \overrightarrow{pool}_k, \overrightarrow{unp}_k, \overrightarrow{res}_k),  \\
%&\forall (n,k) \in [1,N]\times[1,K]\ and\  i\coloneqq n*K+k \Big\}.
%\end{split}
%\end{equation}%
%We can observe the presence of sample sets in four quadrants from Fig \ref{Sample_quadrant}.
%These two lines $q_i$ and $t_i$ divide samples into two sections: (i) $I^{pos}$, i.e., shaded part and (ii) $I^{neg}$, i.e., blank part in Fig \ref{Sample_quadrant}.

%Based on the MLP-based controller, we can quickly reflect the acceptability of different CNN-based approximate models under a specific user metric $U(Q, T)$. Generally, there are several approximate models satisfied users' constraints if the metrics are set properly. After several approximate candidates are selected by the MLP, We develop a runtime algorithm to adaptively select models to achieve the execution time benefits.
%1.model topology.%The MLP model has an output layer with a single node to generate the final estimation. %By training the MLP binary classification model on the enormous training sets and approximate models, we are able to obtain an elaborate MLP that determines the acceptability whether the approximate model is able to process fluid simulation samples with given metrics. %\subsection{}


%\textbf{Effectiveness of MLP-based quality controller.}

%Effectiveness in finding optimal approximate candidates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/Prediction1.pdf}
  \caption{Prediction 1.}
  \label{prediction1}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/prediction2.pdf}
  \caption{Prediction2.}
  \label{prediction2}
\end{figure}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/pipeline.pdf}
  \caption{Pipeline.}
  \label{pipeline}
\end{figure*}

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\textbf{Ensure model accuracy.}
%Use auto-keras.

%\subsection{Selection of Approximation Models}
%\textcolor{red}{Paragraph1: explain why efficiently select the model candidates is important}
%A large amount of model candidates can be generated after Neural Network Transformation, but we find not all of these model candidates have equal performance after adequate experiments. Based on the experimental results in terms of the performance and time cost of these model candidates, we find only a few of them possess high performance and low time cost.  Therefore, how to efficiently select such model candidates and neglect the others is another inevitable challenge.  In this section, we applied single-tenant model selection using multi-armed bandits to address this challenge. Not just apply the existing approach, we also take time cost into consideration during model candidates selection due to model candidates with similar performance may have vastly different time costs.  Efficient model candidates selection can not only improve the performance but also make our framework more accessible and usable for users. 

%
%\textcolor{red}{Paragraph2: illustrate how to efficiently choose the model candidates in our paper(do we also need a pseudo code for it, any suggestion? multi-arm badit argorithm).}
%The model candidates selection problem in our scenario can be defined as follows. For a user with a Eulerian Fluid Simulation application using neural network based approximation, assume there are $n$ possible model candidates we can choose after Neural Network Transformation, the model candidates set can be represented as $\textbf{M} = \{m_1,...,m_n\}$. The input for these candidates are the divergence of the velocity field, $\nabla.u^{\star}_{t}$, and a geometry field $g_{t-1}$, the output is an estimated pressure value, $\hat{p}_{t}$. When the user wants to simulate the Eulerian Fluid using CNN models at time $t$, the input and output can be specified as $input = [\nabla.u^{\star}_{t}, g_{t-1}]$ and $output = \hat{p}_{t}$ respectively. Then our system automatically matches all neural network candidates in $M$ that can be used for simulation. Whenever a model candidate finishes simulation, the system returns the estimated pressure value $\hat{p}_{t}$, then the $\hat{p}_{t}$ will be used for calculating the value for objective function based on Equation \ref{Equ:Objective_function} to calculate the loss value. After this process, the user can observe the loss value for each model candidates at time $t$, $loss_{m_{i},t}$. Then, the best $k$ model candidates that the user selects at time $t$ can be denoted as $\textbf{m} = \min\limits_{k}loss_{m_{i},t}$. The destination of the model candidates selection is to find a sequence of candidates for simulation in order to reach a lower $loss_{m_{i},t}$ as fast as possible. The core of the model candidates selection part is an automatic scheduler that prioritizes the execution of different model candidates for the user. We formalize such scheduling as a \textsl{single-tenant model selection} problem while taking time cost into consideration. 

%\textcolor{red}{Paragraph3: what's the result of our model candidates selection approach compared with the baselines(ICML)}



%\textbf{Model construction results.}
%Figure~\ref{fig:model_construction_results} shows one result after model candidates selection, the red points denote the selected model candidates, the blue points indicate those discarded candidates, x-axis represents the time cost of the candidates, and y-axis is the quality loss. The goal of our model candidates selection is selecting those candidates possess low quality loss and time cost, while discarding the rest of them. In this experiment, 128 model candidates are generated in total after neural network transformation, 15 of them are selected via our model candidates selection approach. Those strong candidates are located in the left bottom corner of Figure 3. As the figure shows, we can find only one candidate with relative high quality loss and time cost is selected by our approach, while those selected candidates either possess low quality loss or time cost, or both of them. This outcome indicates the efficiency and accuracy our proposed model candidate selection approach.  

%Smaller neural network without performance loss is ideal notion for the transformation, therefore, four novel morphism operations are proposed to transform the neural network $\phi \in \Phi$, which can be reflected through the change of computational graph $G$. The first operation is deleting a layer of network $\phi$ to make it shallow and efficient, which denoted as $shallow(G,L)$, where $L$ represents the layer where deleting operation takes place. The second one is narrowing a layer in $\phi$ denoted as $narrow(G, L, r)$, where $L$ is the intermediate layer needs to be narrowed, $r$ is the number of neurons reduced at the layer $L$ which can be either a fully-connected layer or a convolutional layer. The third operation is pooling. Pooling operation $pooling(G, L, m)$ downsamplings the layer $L$ using a pooling matrix $m$. 
%In our case, downsampling the resolution features enable efficiently reduce the image size with relatively lower resolution. The fourth one is dropout. Dropout operation $dropout(G, L, p)$ drops neurons with a given probability $p$. In our case, there are multi-resolution features to enable modeling the fluid dynamic simulation. Dropout operation prevents overfitting and reduces computational complexity without degrading accuracy significantly.

%
%\textcolor{red}{Paragraph3: explain these four operations in detail.} 
%First, the $shallow(G,L)$ operation deletes a layer $L$ in the computational graph $G$ which will generate a new graph $G^{'}$ with less layers. This operation not only shortens the depth of neural network but also reduces the time for initializing the weight, thus it makes the simulation process more efficient. 

%Second, we define an effective area for operation $narrow(G, L, r)$ as $\varphi$ to better describe how to change the network. The effective area $\varphi$ consisted by a set of neurons in the computational graph $G$ which can be recursively defined by the following rules: 1. $u \in \varphi$; 2. $u_{0} \in \varphi$, if $\exists e_{u \to u_0} \notin L_{s}$, $u \in \varphi$; 3. $u_{0} \in \varphi$, if $\exists e_{u_0 \to u} \notin L_{s}$, $u \in \varphi$. $L_{s}$ represents a set of fully connected layers and convolutional layers. Operation $narrow(G, L, r)$ changes two set of layers, the previous layer set $L_{p}=\{e_{u_0 \to u} \in L_{s} \mid u \in \varphi\}$ outputs a narrower tensor, correspondingly, the next layer set $L_{n}=\{e_{u_0 \to u} \in L_{s} \mid u_0 \in \varphi\}$ also inputs a narrower tensor.

%Third, the pooling operation $pooling(G, L, m)$ can reduce the amount of parameters and computation in the network, and hence to also control overfitting. One common form is pooling with matrix $m$ of size $2 \times 2$ which discards 75\% of the activations. Different pooling strategies can be applied during the transformation, like $max pooling$, and $average pooling$ etc. The dropout operation $dropout(G, L, p)$ discards the neurons in the layer $L$ with the probability $p$, this operation will generate a sparse neuron network which leads to less computations for fluid simulation.
%Note that since our network is fully-convolutional, the size of the domain can be modified at inference time. The network can perform inference on any size domain.

%Previous work on neural network transformation is mainly based on two methods: layer-level and graph-level transformation methods. Layer-level transformation preserves the functionality of the layers that operators applied on, while it can violate the input and output tensor shape consistency for the entire network. The graph-level transformation approach was proposed to address this challenge, and existing work generally changes the architecture of neural network by different morphism operations. Therefore, these operations either make the network deeper or widen the intermediate layers which lead to more expansive networks with larger calculations involved. However, fluid dynamic simulation is known as a computation intensive application, such morphisms make them unsuitable for our transformation as they bring more computational burden for the simulation. Based on this drawback, we design four morphism operations based on graph-level transformation to tackle this challenge.     

%
%\textcolor{red}{Paragraph2: include some basic information about these four operations.} %\textcolor{red}{Figure~\ref{fig:Output Quality Variation} shows the result after $narrow$ operation, we can find the output of the previous layer and input of the next layer are reduced through this operation. Therefore, this operation reduces the computation during the fluid simulation process.} %\textcolor{red}{The $max pooling$ means leave the max number in the matrix $m$ and discard the others; the $average pooling$ makes an average for the numbers in the matrix $m$.} 

 %for varying stages and situations.  

%\textcolor{red}{LJ, 1-2 paragraphs:explain four different operations to develop different model typologies.(see paper auto-kares for detail.}
%Plan to use three paragraphs to explain four different operations. 
%
%\textcolor{red}{Paragraph1: clarify the motivation, why we use these four operations.}
%Furthermore, we take time cost into consideration during model candidates selection due to the new generated models with similar performance may have vastly different time costs.

%At the beginning, our framework maintains a basic CNN model as the input for generating an approximate model pool. 
%Unlike transformation approaches in Auto-Keras \cite{jin2018efficient} which suffer from a heavy computational burden to produce a larger neural network, our operations for model transformation like $shallow$, $narrow$, $pooling$, and $dropout$ can generate a smaller neural network while introducing a tolerable performance degradation. Among the obtained large volume of mophism set,  some model candidates may have poor performances.
%Therefore, we have to select the model candidates with a good performance under the time constraint. Here, we regard this challenge as a single-tenant model selection problem while taking time cost of the candidates into consideration. 
%Once the model construction part finished, a model pool will be obtained consisted by some appropriate model candidates which maintain high performance and relative low time cost.%The whole training process of MLP is off-line and the MLP-model can bound quality error and %
%The MLP model will the success rate of a model under given  takes in the user metrics and the configuration of a model to assess this model.%Smart-fluid first selects the highest probability model and pre-executes a short-step simulation, and then the final simulation quality of this model is predicted by the DivNorm collected. A newly designed adaptive algorithm chooses most suitable approximation model by comparing predicted output quality and user requirement and then procedure continues until the end of simulation. 
%
%\textcolor{blue}{WQ: Overview(3-4 paragraphs)}
%Smart-fluidnet is a framework that enables adaptive neural network-based approximation to accelerate Eulerian fluid simulation. The input of Smart-fluidnet includes the user requirements on the final simulation quality and \textcolor{blue}{the execution time of the approximated computation in the fluid simulation}. After applying Smart-fluidnet, the final simulation quality should be no worse than the user requirement and the execution time should be shorter. The input of Smart-fluidnet also includes a neural network model. Note that using a single neural network model to approximate computation has limitations because of the lack of flexibility and generalization, discussed in Section~\ref{sec:intro}. Smart-fluidnet aims to address the limitation in a systematic approach.%smart-fluid is an adaptive approximate framework that dynamically accelerate fluid simulation constrained by user demands. Because multiple CNN-based approximate model candidates expose generalization ability and flexibility and can be effectively chosen by  various input problems. Given a user demand metric, a set of inputs, and a basic approximation model, the goal of our framework Smart-fluid is to quickly choose appropriate approximate models for user requirements and dynamically switch models to fit different inputs. High level work flow of our framework achieving is depicted in Figure~\ref{figure:overview}. The framework composes of three modules, i.e., \textsl{approximation model construction}   (\cref{sec:model_building}), \textsl{offline output-quality control} (\cref{sec:MLP}) and \textsl{quality-aware runtime design} (\cref{sec:lightweight predictor}).

%\textcolor{green}{Rewrite the following paragraph to make it easier to understand.}

%Equation \ref{equ:NS_momentum},%\textcolor{blue}{para 1: Incompressive Navier-Stokes equations}
%Real-time simulation of fluid flow is governed by the impressible Navier-Stockes equations, a set of partial differential equations.
%\begin{equation}
%       \bigtriangledown \cdot \vec{u} = 0
%       \label{equ:Euler_condition}
%\end{equation}
%The two equations are solved in each time step of the fluid simulation 
%adjusts the pressure field at each time step of the fluid simulation 
%In Equation~\ref{Equ:Possion_equation}, $\vec{p}$ is the pressure of the fluid. 
%Equation~\ref{Equ:Possion_equation} is solved


\begin{comment}
Fluid dynamic simulation aims to study the flow of fluid materials and has been widely applied to multiple disciplines including chemical physics, material science, computational fluid dynamics, to name a few ~\cite{de2012computational,choi2018feasible,rutkowski2018surgical}.
% other scientific research fields.to study the fluid flow
%
However, the simulation of fluid dynamics usually requires prohibitively high computational~\cite{xiaparallel,snyder2019cfd} resources and thus limit its application in these related fields.
%is an exceedingly computation intensive application.
In fluid simulation, as the number of grid points increases, the range of length- and time-scales is not only large but also comprehensive.
%
The size of computational fluid simulation problem was growing exponentially~\cite{cant2002high,afzal2017parallelization}.
%
From the report of U.S. Department of Energy, their simulation scale is approaching Exascale order now~\cite{nielsen2018scaling}.
%
The simulation scale is so massive that the computational overhead is unbearable.
%The state of an target fluid system are described with an  equation, which is highly complex and cannot be analytically solved.
Navier-Stokes (N-S) equations governing fluid flow are highly complex and cannot be analytically solved.
%
To this end, we use numerical methods such as Preconditioned Conjugate Gradient (PCG) algorithm to iteratively solve non-linear partial equations derived from the N-S equation.
%
However, N-S equation is symmetric and positive semi-definite with a large number of free parameters.
%
%To solve the N-S equation in Fluid simulation, conventional convex algorithms are strongly data-dependent and involves unpredictable computation overhead. 
%
%To exhaust the final convergence, traditional exact solutions such as PCG method suffer from high computation overhead and time cost.
%For example, in a high resolution ($512^3$) smoke and free surface simulations, PCG method uses 395 times iteration and $6648.68 s$ produce an small residual less than $1e^{-8}$ ~\cite{}.  
%
Over the past decades, there is a growing interest in seeking more efficient algorithms to alleviate resource strain.
\end{comment}
%In this part, we briefly list some basic performance information of current mainly used approximation models and analysis their limitations. These information includes the running time and average quality loss for these three mainly used approximation models.
%As the table 1 shows, we measure 20480 samples to test the performance and accuracy of three different methods. PCG has the lowest average quality loss and the longest running time among these three approaches.   Its advantage is the lowest average quality loss, however, the short running time outweighs the low quality loss during the approximation in fluid dynamic simulation, because users care more about running time while a certain extent of performance degradation is acceptable. 
%For instance, the short running time outweighs the low quality loss during the approximation in fluid dynamic simulation.  
%%Thus, this limitation makes PCG unsuitable for approximation in fluid simulation. The approach proposed by Tompson improves the running time for orders of magnitude compared with PCG method. Though its average quality loss is acceptable for approximation, the running time is still too long to be well applied into fluid simulation, as it is highly computation intensive and time constraint. Compared to the previous two methods, the approach proposed by Yang achieves the trade off between running time and average quality loss for approximation. However, this large average quality loss may influence the performance too much for the simulation which makes this method unusable for those users have high simulation quality requirement. 

%For a given approximation model, the output quality fluctuates based on different inputs as Figure ~\ref{fig:Output Quality Variation} depicts.  In Figure ~\ref{fig:Output Quality Variation}, the horizontal axis is the quality loss, and the vertical axis represents the proportion of inputs that can satisfy the users' requirement.  For example, if the users need the quality loss less than $0.01$, the proportion of inputs that will success is 34.58\%, the additional value of the left four columns in the Figure ~\ref{fig:Output Quality Variation}. Therefore, we can conclude that only a part of the inputs can satisfy the users' requirement under the specific quality loss constraint. Based on such limitations of the current work, an approximation approach for simulation with both shorter running time and lower quality loss is indispensable. 



%%%%%%%%%



%From the result of Figure ~\ref{fig:Output Quality Variation}, we can see the output quality variation.
%
%If users want output quality loss less than $0.01$, the success rate based on the proportion is 34.58\%.
%
%Even loose the output quality loss to $0.02$, the success rate is only 79.93\%.


 %ConvNet is one of the most popular Deep Neural Networks (DNNs) organized in a directed acyclic graph where each node is a processing element that applies a function to its input and generates an output. In \textcolor{green}{cite}, the authors approximate the pressure $\hat{p}_{t}$ value in Eulerian Fluid Simulation through a appropriate ConvNet architecture. 
%\textcolor{green}{(pros and cons of different ML algorithms)}

%%After solving the Equation ~\ref{Equ:Possion_equation} to satisfy imcompressible condition, the pressure $\vec{p}$ updates the next time step velocity $\vec{u}^{n+1}$ in Equation ~\ref{equ:NS_momentum}.
%In this paper, we use marker-and-cell (MAC) grids\cite{harlow1965numerical} to discretize our fluid distribution. The computation domain is divided into a fixed rectangular grid with a Cartesian coordinate system. Hence, Equation \ref{Equ:Possion_equation} refers to a large-scale sparse linear system $A\vec{p_{t}}= \vec{b}$ based on MAC grids. As a Poisson equation, the linear system involves a large number of free parameters. The solving process also involve a large amount of iterative computations to converge to a relatively small residual in traditional numerical methods, such as PCG method. Meanwhile, the iterative process is highly computational intensive and hard to estimate its computation overhead.
%To fairly evaluate the accuracy of fluid dynamic simulation, we calculate the difference of density matrix with real-world fluid data as our quality loss by

%As $\rho$ and $\rho_{*}$ are large matrix, we calculate the mean value of their absolute error.  
%In this paper, we use Convolutional Neural Networks(CNN) to accelerate the solving process of Poisson equation. 

%In this paper, we aim to accelerating the linear projection which is the most time-consuming step of fluid simulation.%In the approximation, a certain extent variation for the output is acceptable and some degree of quality degradation is tolerable. Neural Network based approximation means the result of an intensive computation can be replaced by the output of the neural network. Due to some common bottlenecks of traditional approximations can be alleviated by neural network based approximation~\cite{ml_fft}, thus, it has been widely used into some domains such as physics, material science, and computational fluid dynamics. 

%Using a neural network for computation approximation, the original computation and neural network use the same input dataset, and are expected to g. %%%%In this paper, we use Convolutional Neural Networks (CNN) to approximate computation. %CNN is a type of  neural networks that automatically infer features from raw data in order to accomplish tasks such as image classification or object detection~\cite{racah2017extremeweather}. CNN can be used in either supervised (data with labels) or unsupervised (data without labels) way, and in both cases, it is represented as a Directed Acyclic Graph (DAG) consisted by neurons with parameters called weights.%These weights are arranged in layers and number always in the millions, 
%%so as to back-propagate gradients to update those trainable parameters.
%
%\textcolor{green}{Explain what is the objective function here.}

%For each mini-batch, CNN computes a set of scores by performing numerical computations using the model weights, called the  \textsl{forward pass}. Based on the desired task, a specific objective function is designed to measure the divergence between computed score and desired value. This divergence (known as error) is calculated through a backward pass over the model, each forward-backward pass is called a \textsl{mini-batch iteration}. 

%During the training, each mini-batch iteration typically involves millions to billions of floating point operations. Typically, millions of such iterations are performed on large datasets to achieve high performance.
%


%%%%%%%
%Therefore, it is usually used in some domains that are amenable to trade off between performance and accuracy .
%There are many domains where it is acceptable to use approximation approaches.
%
%Machine learning-based approximation is in essence approximate computing.
%We study machine learning-based approximation rather than other approximate computing approaches because it has big advantages over other approximate computing approaches.

%
%There are several 
%
%First, conventional approximate approaches, such as loop perforation~\cite{sidiroglou2011managing, 5470469}, random task discarding~\cite{Rinard:2006:PAB:1183401.1183447}, and synchronization relaxation~\cite{Rinard:2007:UEP:1297027.1297055, Campanoni:2015:HRP:2738600.2738630}, have specific constraints on code structures. 
%
%The requirement could be a loop structure, a task-based execution model, or a communication synchronization. 
%
%Neural Network-based approximation provide a more general approach to adopt various application structures and inputs. \textcolor{green}{(prove your conclusion by cite reference or experimental data)}
%
%Second, Common approaches are generally not cognizant of the hardware it based on and hard to exploit the underlying hardware benefits. \textcolor{green}{cite}
%Neural Network-based approaches are well designed for affordable and powerful GPU engines.\textcolor{green}{cite}
%These methods are more willing to improve computation performance through slightly modification without hurting its original structure instead of an earth-shaking change.
%
%Moreover,  Neural Network-based approaches \textcolor{green}{cite} provide a more transparent and transplantable way for users to implement and tune most aspects of approximation.\textcolor{green}{cite}
%
%need rephrase
%Third, Conventional approximation is hard to provide a certain time cost and accuracy estimation.
%difference between the output and ground-truth
%CNN has been proved to be a powerful regressor for approximating a real number~\cite{george2018deep}. In our case, the Poisson Equation is highly computation intensive and hard to estimate its cost~\cite{pmlr-v70-tompson17a}, while neural network based approximation can provide flexible computation budget and relatively reliable quality control~\cite{richard2014artificial}. Therefore, we construct a CNN to approximate the pressure $\vec{p}$ by importing velocity divergence in an unsupervised way. 

%The input of CNN are the divergence of the velocity field, denoted as $\nabla.u^{\star}_{t}$, and a geometry field, represented by $g_{t-1}$.
%Then the output $\hat{p}_{t}$ is an inferred pressure calculated as follows:  
%\begin{equation}
%\label{equ:CNN_objective_function}
%\vspace{-5pt}
%    \hat{p}_{t} = f_{conv}(W,\nabla.u^{\star}_{t},g_{t-1}).
%    \vspace{-5pt}
%\end{equation}
%Where $W$ is the parameters to be optimized by the objective function $f_{conv}$ using ADAM~\cite{Kingma2015AdamAM} optimization algorithm in our work.

%During the training process, $DivNorm$ is minimized during the training and used for evaluating the model loss in the inference phrase.%\textcolor{green}{(why $\vec{u_t}$ is predicted? It is input, right?)} 

%\textcolor{green}{Simplify the following paragraph, because we already discuss some points in the overview section. Some of the following paragraph can be moved to the overview section.}
%\textcolor{red}{simplified:}%without comparing with the ground truth. Note that we take PCG method as a ground truth in this paper. %approximation model candidates loss $DivNorm$ and simulation loss $Q_{loss}$%\textcolor{green}{(Simplify the following paragraph. Many points in the following paragraph have been repeatedly discussed.)}
%After selecting some promising candidates by the MLP controller, we use these approximation model candidates to accelerate simulation at runtime. There exists a problem that how to build a calibration for appraising multiple approximate candidates at runtime that can be used to predict the quality loss $Q_{loss}$  and guide fluid simulation.
%In general, a relatively small quality loss $Q_{loss}$ should be guaranteed during fluid simulation and is represented in Equation~\ref{eq:quality_loss}. 
%\textcolor{red}{revised.}%and it is impossible to evaluate which approximate model is optimal. %During the exploration stage \textcolor{green}{(what is ``exploration stage''? You never define it)}, %    \item \textbf{Observation 3}: %\textcolor{red}{$Q_{loss}$ never decreases. Even we switch to the exact method, it still turns to a `flat' stage (a negligible increase).} %\textcolor{green}{(rephrase the above sentence. The english is too difficult.)}%\textcolor{green}{(do we have a figure to support the above observations?)}  

%\textcolor{red}{Based on these observations, we conclude that the accumulated $DivNorm$ may related to $Q_{loss}$ or has a similar increasing tendency.}

%\textcolor{green}{(What is "loss"? Do we explicitly define it somewhere before this section?) Rephrase this sentence. The english is difficult.} 
%As shown in Equation \ref{equ:cundivnorm}, the cumulative $DivNorm$ of the $n{\text{-th}}$ timestep is expressed as follows ($n$ is the last time step):
%In order to validate our assumption and more accurately show the possible connection between $CumDivNorm$ and the final $Q_{loss}$, two widely employed indicators, the Pearson's product moment correlation coefficient ($rp$) and the Spearman's rank correlation coefficient ($rs$), are used to reveal statistical relationship between two factors. The $rp$ is a measurement of the strength of linear association and $rs$ is the nonparametric version of the $rp$. The largest distinction between these two statistical indicators is that $rp$ only measures linear relationships while $rs$ is only for monotonic relationships. %\textcolor{green}{(What is the pairwise distance? What is the rank? Cannot we use simple language to explain them?)} A larger value of $rp$ or $rs$ indicates a stronger relationship.

%$x_i$ and $y_i$ are \textcolor{green}{xxxx}; $d$ is \textcolor{green}{xxxxx. Do we need to explain d here?}. 
%\textcolor{green}{(Why 0.67 and 0.73 can show strong correlation? Do we have any reference?)}
%Test results on 20480 samples show that Pearson's correlation is 0.67 and Spearman's correlation is 0.73, and then the strong correlation is proved between $CumDivNorm$ and $Q_{loss}$. %The loss of model $DivNorm$ always be accumulated and will affect the final simulation loss in fluid simulation.  
%During fluid simulation, performing accurate approximate models will loss the opportunity to accelerate the simulation while using a coarse approximate model may lead to unknown quality violation.
%%Based on the above conclusion on the correlation between $CumDivNorm$ and the final quality loss, we can use $CumDivNorm$ to predict $Q_{loss}$.
%during runtime.we observe the $DivNorm$  and try to predict final $CumDivNorm$ with minimal overhead.
%\textcolor{red}{%\textcolor{green}{(Is this a new observation we should put into the observation list? We don't mention anything about this observation before this point)}, %and further improve the prediction accuracy using exponentially weighted loss values. %(\textcolor{green}{(what is the ``loss values''?)}) 
%Intuitively speaking, $CumDivNorm$ obtained in the near past are more informative for predicting final $CumDivNorm$.
%The weights assigned to history data decay exponentially when new timesteps finish, and the parameters of the curve equations get adjusted for each prediction. \textcolor{green}{(the last sentence is confusing. How does the last sentence connect with the rest of the paragraph? What is the logic flow? Confusing)} %At runtime, we dynamically fit a linear curve $f_{k}(x) = ax + b$ of $CumDivNorm$, where $x$ is the index of timestep. This curve is used to predict final $CumDivNorm$ using the least square method based on historical data and further designed to improve the prediction accuracy using exponentially weighted loss values. Intuitively, loss values $CumDivNorm$ obtained in the near past are more informative for predicting final $CumDivNorm$. The weights assigned to history data decay exponentially when new timesteps finish, and the parameters of the curve equations get adjusted for each prediction.%\textcolor{red}{where $n$ is the timestep of .} %\textcolor{green}{(why "current"? What does it mean?)}
%\textcolor{green}{wenqian : please modify the previous paragraph!!!}

%\textcolor{green}{The below paragraph needs to be polished.}
%When switching to another approximation model at runtime, we take previous $CumDivNorm$ as a constant \textcolor{green}{(why does the above sentence mean?)} and add to a new fitting curve. The predicted $CumDivNorm$ dynamically changes according to the fitting function $f_{k}$ at each timestep.  
%\textcolor{green}{wenqian : please modify the previous paragraph!!!}
%(Cannot we just directly introduce linear regression method? This paragraph is not used later.)%Therefore, we introduce the K-nearest neighbors (KNN) method to reveal correlation-based matching, which can be used to reliably reflects the final quality loss. %\textcolor{green}{(training phase? The training phase to select the neural network?)}

%\textcolor{green}{(The last two sentences are confusing. I cannot understand.)}%\textcolor{green}{(what is "pairs"?)}
%by calculating the distance between the $CumDivNorm$ of historical data and $CumDivNorm'$, e.g., 0.09-101, 0.11-112 0.10-105, 0.11-109 and 0.12-113, and take the average 0.01 as the predict $Q_{loss}'$.  %and the relatively simple calculations bring almost negligible overhead.%Smart-fluid uses the most promising approximate models predicted by the MLP-based controller to maximize the benefits of performance and accuracy.
%For a user given quality loss $Q_{loss}$, we get a target $CumDivNorm^{tar}$ using the KNN algorithm and use it to adjust our app proximate candidates.
%The detailed algorithm of the Smart-fluid is depicted in %\textcolor{red}{(Why do we use ``flops''? The execution time can be directly measured during the model training time, right? rephrased.)} 

%It is worth noting that these candidates can meet the user requirements with a certain confidence, which equals to the given possibilities of MLP-based controller.%run the recommended model with the highest possibility and % at the simulation end frame \textcolor{green}{(what is the simulation end frame? is it the last time step?)}; %in an acceptable error ($\pm 5\%$) ($Q_{loss}'$ < $Q_{loss}$) (\textcolor{green}{Why do we have an error tolerance 5\%? Can we remove 5\%?}), %\textcolor{red}{requirement,} %\textcolor{green}{(what is the threshold? 5\%?)}, %the highest probability among available candidates and  continue switch to coarse approximate models until finding the suitable one. %\textcolor{red}{(lower? Did we just discuss the lower case? Why do we consider the lower case again? yes, that is why we can guarantee the simulation quality.) }%a one that is higher than the flops of the current model with the highest probability among available candidates, and continues the simulation%In addition, if all approximate models are unable to meet quality demand, we restart the calculation and solve this equation by the exact method. 
%shows an example adaptively selects an optimal approximate model over five candidates.
%Given a user metric U(0.013, 6.64s) and an input sample with the grid of 1028*1028. In Step 1, we collect five approximate models by MLP-based controller and mark the computation overhead using its execution time. Then we pre-execute the approximate model $M1$ which has the highest Probability (91\%) in Step 2. As Step 3, We fit the $CumDivNorm$ curve of $M1$ and get its predicted $Q_{loss}'$, i.e., 0.019. As described in Step 4, the predicted $Q_{loss}'$is lower than expect, then we switch to a more accurate approximation model, i.e., $M3$ (a model with longer execution time and maximum probability among available candidates). For $M3$, the predicted $Q_{loss}'$ is 0.015 by the five closest records. We repeat the operation above and switch to $M5$, then the predicted $Q_{loss}'$ is 0.13, which achieve user target. So we find the optimal approximate model $M5$ and continue use it in following steps.

%As shown in the current example, since predicted output quality of M1 model cannot meet user's requirements, then the M2 model is reselected and the Step2 and Step3 are performed, and equation is finally solved using M2 model that meets requirements. 
%A major premise for the runtime system is a set of appropriate models that are used to build a quality-aware model-switch system. The interface of the runtime system is mainly composed of two parts based on Inspector-Executor method. The inspector briefly pre-executes model, predicts the output quality that the model can achieve, and choose the fastest and most accurate model that meets the requirements. The executor solves the entire equation by reusing predicted result. With the number of time step increases, these overheads are almost completely diluted and the proportion of overhead will be greatly reduced.

%\textbf{Discussion.}
%\textcolor{green}{We need to add a discussion on the limitation of the above runtime algorithm. I think the limitation is that the runtime system needs to take some time steps to find the optimal neural network model. The process of finding the model could be time-consuming. But we can argue that our model candidates are a few and it usually takes ~10 time steps to find the best model.}

%
%Given an assumption that during runtime, we use the most accurate model in \textit{Appr. Model Pool} to revise some inputs which can't achieve user time constraint $t_u$ using the current approximate model $M_k$.
%After the acceptability probability of an approximate model $\rho_{suc}$ is evaluated by MLP, we calculate the total running time using $M_k$ based on the above assumption.

%Since the training of our models requires sufficiently large computational resources, we equip the server with an NVIDIA Titan X (Pascal) GPU card, which helps accelerate the fluid simulation fundamentally.The GPU card consists of 3,072 CUDA cores running at 1.0GHz.%we choose various grid sizes including 128$\times$128, 256$\times$256, 512$\times$512, 768$\times$768, 1024$\times$1024. Here, the grid sizes represent that how many vertical and horizontal pixels are captured to make the matrix of a fluid state at certain timesteps.%all the generated models are re-implemented and optimized in the Torch7 package, which is a scientific computing toolset. %written for Lua.
%
%The other part of fluid simulation are also implemented in Lua, which enables us to go through all the experiment smoothly.
%We also implement the proposed discriminative MLP model and runtime algorithm in Lua/Torch.
%%The proposed discriminative MLP model and runtime algorithm are also implemented in Lua/Torch.
%
 
%(Target quality and Time cost limitation)
%\noindent\textbf{User Metric}.
%In different practical scenarios, users may have specific quality requirements and execution time limitations.
%
%To be fair, all experiments in this evaluation use the average execution time and average quality loss as user metric $U(Q,T)$. 
 %\textcolor{blue}{deleted}
%\textcolor{green}{The above two sentences are confusing. Can we delete them?}


%to evaluate other algorithm's superiority in terms of processing speed and accuracy.

%The speedup $S$ of a fast algorithm such as Tompson's or our proposed method is calculated as follow:
%\begin{equation}
%    S_{fast} = \frac{T_{PCG}}{T_{fast}}.
%\end{equation}

%We show the results of our algorithms compared with Tompson's method in terms of speedup in Figure ~\ref{fig:Speedup}.
%In this figure, it can be observed that our proposed framework ``Smart-fluid'' performs favorably against the Tompson's method under different grid settings. %\textcolor{red}{To be justified with experiments}. %With the grid size of 256$*$256, the speedups of  Tompson's method and Smart-fluid are 560.88$\times$ and 620.80$\times$. While with the grid size of 1024$\times$1024, the speedups are 273.30$\times$ and 467.16$\times$ respectively. Overall, in different grid sizes, our method obtains higher performance advantage against Tompson's in terms of speedup.%user target(0.01,Tompson average time and average quality loss for each different input )
 
%To make fair comparisons with Tompson's algorithm, we take these two values as baselines to generate reasonable user metrics. Specifically,  we choose 0.013, 0.015, 0.015, 0.012, 0.013 as the target quality loss and choose 0.240, 1.45, 2.97, 3.82, 6.64 seconds as the target time cost for the grid size settings of 128*128,256*256, 512*512, 768*768, 1024*1024 respectively(\textcolor{red}{need a table? too many figures and tables in this para).}
%user demand time is xxx s, xxx s,... for form statistical data of ....


%We present the boxplot in Figure~\ref{fig:sec7_2} to show the output quality of both methods across different input problems. The central mark indicates the median, and the bottom and top edges of the box indicate the 25-th and 75-th percentiles, respectively. The whiskers outside a box indicate the minimum and the maximum, while the `+' markers represent the extreme outliers. With the grid of 128*128, our results have relatively tight boxes than the Tompson's, which indicates a smaller variation of quality loss. Although the Tompson's methods achieves the user target on average of the evaluation dataset, there are quite a lot inputs suffering large quality loss especially, as implicated by those extreme outliers. In contrast, the quality loss of ours is more compact under the target line 0.013, which means that our method can achieve the user demands sufficiently but without too much too much quality violation, \textcolor{red}{11.75\% too high???}. When we examine the other grid size settings, similar findings can be obtained that our method can achieve user demands even when the samples might largely vary from one to another. Our method is less sensitive to different input samples than Tompson's. We generate less wild outliers than Tompson's method.

%Accuracy of handling different samples.%In Table \ref{tab:success rate}, we present the ratio that how many samples can achieve the final target. For these input problems, we dramatically improve the success ratio of samples that that satisfy the user demand quality requirement for the grid size form 128 to 1024. Smart-fluid works very well at dynamically choosing a optimal approximate model on accelerating and reduce quality violations in practice. However, we note that Smart-fluid makes no 100\% guarantees about output accuracy. In other word, we can generate more accurate approximate models for extreme outliers to guarantee final output quality with losing runtime benefit in some extent.

%\textcolor{red}{Do we still need the figure to show quality loss of each timestep?
%figure xx(pending): quality loss with timestep (our framework VS google model VS PCG);
%(average quality loss for each timestep?)}

%%We analyze the effect of using different switching steps as required by runtime algorithm.
%As the switching of models requires additional time consumption to the runtime but may brings in higher accuracy when the user demand is rigorous.
%%The adaptive algorithm requires additional time consumption to the runtime to bring higher accuracy when the user demand is rigorous.%As is shown in the Figure~\ref{fig:sec7_7}, when the switch stride varies from 2 to 20, the overhead drops down from 0.24 to 0.06 seconds. Furthermore, we define the accuracy as the success rate of how many samples reach user target. In Figure~\ref{fig:sec7_7}, it is observed that the accuracy drops from 86.5\% at point 4 to 43.67\% at point 18 with fluctuations.

%\textcolor{red}{Need more details?}
%A larger stride may reward us a more appropriate approximate model. While a frequent switching will help the online adaptive algorithm seek for accurate models more aggressively because of a lack of full knowledge about the efficiency of current approximate model on the current input sample. From the figure, we suggest that using a switch stride between 4 to 8 is  a good trade-off of the overhead and accuracy for the fluid simulation by our runtime algorithm.

%\textcolor{blue}{(can we a table to show how frequently each of the 14 models is selected by smart-fluid?) I think the following paragraph seems should put into sec7.3)}%
%\textcolor{blue}{(Do we have the execution time (speedup)? }

%To compare their performances on execution time, we test both the execution time with or without MLP.%The baseline is to replace the MLP model with a non-learning based strategy as the runtime algorithm. Specifically, for this strategy, we use the smallest approximate model candidate and switch to an accurate one until we reach the user requirement by exhaustively searching all available candidates.


%In Figure~\ref{fig:sec7_6}, we compare the variation of the quality losses for all evaluated samples between using the MLP-based quality controller and the exhaustive search strategy. The results show that our proposed MLP model being the runtime controller can achieve higher accuracy under different grid size settings. Here, the accuracy is defined as the success rate that how many generated samples reaches the user demands.
%The variation of the quality losses for all evaluation samples are compared \textcolor{red}{more details? We've got too many results.}
%%online adaptive algorithm Similar to the previous analysis for our framework, we investigate the performance on both the speedup and accuracy metrics.

%In this experiment, we take the Tompson's method as the baseline to calculate the speedup of other methods.
%\begin{equation}
 %       S^{\prime}_{other} = \frac{T_{Tompson}}{T_{other}}.
%\end{equation}
%
%As the Tompson also uses CNN layers to construct their efficient model and our generated model candidates may have deeper layers than theirs, the $S^{\prime}$ might obtain smaller than 1 value.
%Namely, the speedup refered in this section does not represent its original meaning as in previous section.
%
%Tompson:as the speedup baseline;
%1)compare with ICML google model;
%\textcolor{green}{(Don't change the baseline. change the above paragraph.)}%In Figure~\ref{fig:sec7_4}, we show the speedup of different models, including the each of the generated 14 models by AutoKeras, and the integrated Smart-fluid model. We observe that some of the available candidates may not be as fast as Tompson's, the proposed Smart-fluid can process the evaluated samples with providing relative speedup. This demonstrate that our proposed runtime algorithm is able to gain acceleration margins when making trade-offs between efficiency and accuracy during the fluid simulation.
%%In Figure~\ref{fig:sec7_5}, we show the boxplots of the 15 evaluated approximate model candidates and our Smart-fluid algorithm on the dataset. As can be found that for each of the 15 candidate models, there exists quite a large number of outliers outside the boxes. This phenomenon justifies our concerns about the insufficiency of one single model fitting various input samples. However, with different models that are capable of dealing different kinds of samples, our proposed runtime algorithm could adaptively select the appropriate one to deal with each specific sample. The boxplot of our Smart-fluid algorithm generate much smaller amount of outliers and most of the samples satisfies the user demand of lower than 0.01 quality loss. \textcolor{green}{(where does "0.01" come from?)}

%11:different approximate model candidates accuracy(quality loss variation)).%Recently, fluid simulation have attracted extensive interest among several different research fields including physics, chemistry, and computer graphics. %Since the emergence of Deep Neural Network (DNNs) as a prominent technique in the fluid simulation and different super computing settings are at hand now, some researchers put their efforts to apply DNNs to address problems faced in the fluid simulation process. %\textcolor{green}{The above sentence is a little confusing.}%a DNN is trained using the output from simulations and then used to learn the dynamic behavior of the heated line. 
%Moreover, the NN models enable online control and fast assessment of the dynamic thermal-hydraulic system.%Such characteristics make multi-grid approach unsuitable for applications involve intensive computations. %%However, these proposed approaches may not be effective in big data scenarios as fluid simulation involves both low latency and high performance.%The NN-based approach exceeds the best traditional methods in accuracy (95\% v.s. 85\%).
%2.ML become a promising method, describe the details; Introduce the advantages of this method, and define the state of the art [xx]. 
%Neural network based approximation as an efficient and robust way to provide fixed time cost and deliver strong portability on exploiting GPU devices has shown preliminary success.
%
%in some HPC problems such as \textcolor{red}{matrix decomposition? particle simulation?? some examples}~\cite{esmaeilzadeh2012neural}(???). 
%
%For example, Radovic~\cite{ichep16:radovic} proposes to detect neutrinos using a convolutional neural network and achieved a 49\% improvement on signal-detection-optimized efficiency; Wigley et. al~\cite{sr15:widley} achieve Bose-Einstein Condensates state in only 10-12 experiments with neural network which is 10 times faster than traditional models that require 140 experiments. instead of 140 experiences using which reduces the simulation time by 10 times. Other successful examples of using neural network for HPC applications include recognizing extreme weather events in large-scale climate simulations~\cite{nips17:racha}, and medicine prediction for cancer~\cite{candle_anl}.



%%In the context of neural network based approximations for fluid dynamic simulation, Tompson et. al ~\cite{tompson2017accelerating} providing the long-term stability under a fixed computational budget.%\textcolor{green}{(Wenqian, add a few references here (not just one).)}%Neural network based approximation are also able to accelerate fluid simulation \textcolor{red}{while or by???} 
%some of the intermediate layers to delete these layers. This operation will be stopped when a significant performance reduction observed. %Therefore, the value of the $r$ should be less than $\frac{|L|}{2}$. For guaranteeing the performance of new generated neural networks when applying the previous two operations, we test the result of the transformation to avoid significant performance reduction. %the $dropout(G, L, p)$ operation is applied to delete each neuron in intermediate layers with the probability $p$, where $p \in [0,1]$. The new generated neural networks may have a good performance during training, but they may not perform well for testing. Thus, another destination of the last two operations is avoiding overfitting for the new generated neural networks. 
%The goal is selecting these model candidates while discarding the others. We use the \textit{Pareto optimality} method to find these points. As the Figure~\ref{fig:model_construction_results} shows, 128 model candidates are generated in total after neural network transformation, 14 of them are selected via our approach. We can find those strong candidates with low quality loss, low time cost, or both of them are selected, while the rest of them are discarded. This outcome indicates the efficiency and accuracy of our model candidate selection approach.
   
%The quality control requires that the success rate should be aware when using a selected neural network model under restricted user requirement.%based on the user requirement and given the new models after model construction,
%\textcolor{blue}{Specifically, we design an MLP-based quality controller to choose models for online approximation.} 
%to reflect the characteristics of neural network models facing different input problems. 
%We use the tuple as metric $U(Q, T)$ which is customized to guide the following simulations. The $Q$ represents the quality criteria and $T$ stands for time limitation. Based on the metric, we design an MLP-based quality controller to reflect the characteristics of neural network models facing different input problems. %%We propose a prior profiling mechanism to describe the process of training samples collection for the MLP-based quality controller.
%As MLP is used to distinguish neural network models which are suitable to meet the user requirement, then the training samples of MLP must reflect inherent properties of neural network models, i.e., time cost and final quality loss.
%A simple and efficient approach to generate training samples is using the profiling results of neural network models. %which needs to discriminate the most suitable neural network models.%%\noindent\textbf{Training Sample Construction.}
%Finally, we further generate the input of training samples by combining with the properties of neural network models. The efficiency of an neural network model $M_k$ is highly related with the hyper-parameters of network architectures, such as 

%
%We construct a positive set $I^{pos}$ and a negative set $I^{neg}$ by combining with these parameters, which are shown in Figure~\ref{fig:MLP_model}, %
%The acceptability is high when the $\hat{r}_{n,k}$ is close to 1. %To train the MLP model,
%At the same time, our MLP model evaluates the acceptability probabilities of available neural network models. 
%A larger output value by the MLP-based quality controller reflects higher acceptability to achieve the user's expectation, i.e., the success rate of input problems.
%Let $\rho_{suc}$ denote the success rate of a selected neural network model $M_k$.

\begin{table}[!t]
\centering
%\footnotesize
\caption{\textcolor{wq}{MLP Candidates with different typologies.}}
\vspace{-8pt}
\label{tab:success rate}
\begin{tabular}{l p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{1.2cm}}
\hline
Models & $MLP_1$ & $MLP_2$ & $MLP_3$ & $MLP_4$ & $MLP_5$ \\
\hline   
Top-1 acc. & 68.2\% & 76.6\% &89.20\% &91.0\% & 90.8\%\\
Top-5 acc. & 88.2\% & 89.4\% & 91.36\%& 91.47\%& 91.05\% \\
\hline
\vspace{-20pt}
\end{tabular}
\end{table}

==> template_old/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> template_old/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
